DiDOTS: Knowledge Distillation from Large-Language-Models for Dementia Obfuscation in Transcribed Speech

Dementia is a sensitive neurocognitive disorder affecting tens of millions of people worldwide and its cases are expected to triple by 2050. Alarmingly, recent advancements in dementia classification make it possible for adversaries to violate affected individuals' privacy and infer their sensitive condition from speech transcriptions. Existing obfuscation methods in text have never been applied for dementia and depend on the availability of large labeled datasets which are challenging to collect for sensitive medical attributes. In this work, we bridge this research gap and tackle the above issues by leveraging Large-Language-Models (LLMs) with diverse prompt designs (zero-shot, few-shot, and knowledge-based) to obfuscate dementia in speech transcripts. Our evaluation shows that LLMs are more effective dementia obfuscators compared to competing methods. However, they have billions of parameters which renders them hard to train, store and share, and they are also fragile suffering from hallucination, refusal and contradiction effects among others. To further mitigate these, we propose a novel method, DiDOTS. DiDOTS distills knowledge from LLMs using a teacher-student paradigm and parameter-efficient fine-tuning. DiDOTS has one order of magnitude fewer parameters compared to its teacher LLM and can be fine-tuned using three orders of magnitude less parameters compared to full fine-tuning. Our evaluation shows that compared to prior work DiDOTS retains the performance of LLMs achieving 1.3x and 2.2x improvement in privacy performance on two datasets, while humans rate it as better in preserving utility even when compared to state-of-the-art paraphrasing models.

==> Sections/discussion_submitted.tex <==
\section{Discussion}
\label{sec:discussion}

\vspace{0pt}\noindent\textbf{Application.} Our proposed system aims to prevent the leakage of the dementia attribute in transcribed speech and safeguard individuals from potential discrimination, such as insurance denial, employment bias, or financial profiling. It can be integrated into healthcare systems, online and mobile platforms, or transcription services to ensure privacy protection for individuals with dementia. We believe that our approach can further promote ethical data handling, and facilitate privacy-preserving communication. 

As a concrete example, consider Android's \texttt{SpeechRecognizer}~\cite{androidSpeechRecognizer} which is being utilized by a large proportion of popular mobile apps (see Section~\ref{sec:motivation}). Google who manages the Android Open Source Project, or other OEMs who built on top of the vanilla version of Android, can modify the \texttt{SpeechRecognizer} functionality to return obfuscated transcriptions to the requesting apps be default. This modification can happen on both the server side or on the mobile side inside the \texttt{speech} framework whenever the results are ready, to handle speech recognition results from both remote and on-device system ASR models. Strategies like using SELinux for Android or introducing dangerous permissions  can ensure controlled access to raw transcriptions by trusted apps while protecting privacy. However, addressing threats from apps accessing audio directly for transcriptions may require further research into novel audio obfuscation methods.

\ignore{
As a concrete example, consider Android's \texttt{SpeechRecognizer}~\cite{androidSpeechRecognizer} which as we showed it is being utilized by a large proportion of popular mobile apps to get access to speech transcriptions. Google who manages the Android Open Source Project, or other OEMs who built on top of the vanilla version of Android, can modify the \texttt{SpeechRecognizer} functionality to return obfuscated transcriptions instead of the originally derived ASR transcriptions to the requesting apps be default.Our text obfuscation can be applied on the server side where the current ASR system for the \texttt{SpeechRecognizer} functionality lies, to obfuscate the output of the ASR system before populated. Alternatively, the modification can be integrated also on the mobile OS side inside the Android's middleware \texttt{speech} framework whenever the ASR results are ready, to handle speech recognition results from both remote and potential on-device system ASR models. 

To allow full utility for trusted apps, the OS provider could follow two strategies: (a) using SELinux for Android to enforce mandatory granted access to APIs accessing original transcriptions only for trusted system apps, or (b) introduce a dangerous permission for accessing raw transcriptions which requires user interaction to be granted. In the former case, all third-party apps would be consider untrusted and won't be able to access raw transcriptions unless a more flexible SELinux for Android version is introduced similar to the design introduced by Demetriou et al~\cite{DBLP:conf/ndss/DemetriouZNLYWG15}. In the latter case third-party apps can also access raw transcriptions but the user will have control over which apps would be granted access to them as the apps will have to explicitly request the new permission. 

Tackling threats from apps accessing audio directly with the purpose of performing the transcriptions themselves requires more careful design to ensure real time performance. A possible approach would be to obfuscate dementia directly on audio. For example, Woszczyk et al~\cite{woszczykInterpseech24} proposed promising techniques for disentangling identity information from dementia in audio and future work could focus on improving its performance for real time applications. 
}
%\textcolor{red}{TODO: Explain how this can be integrated in the Android OS Speech Recognizer; Careful that Google announced Gemini Nano coming in its AI Core. Also, unfortunately, we do not have a proper implementation and evaluation taht we can report on so this might raise even more questions.}


\vspace{5pt}\noindent\textbf{Limitations.} In this work, we perform an in-depth analysis of LLMs' ability to obfuscate sensitive attributes like dementia and demonstrate the feasibility of distilling their knowledge into a smaller, fine-tuned student model. While our main focus is on dementia, our framework can extend to other attributes such as age, emotion, authorship, and gender. our PEFT approach allows for the easy sharing of adapter weights for each attribute, depending on the specific use case. However, due to the difficulty of accessing dementia datasets, our work relies on only two datasets with the same task which restricts the generalizability of our findings. The data may not fully capture the diverse characteristics and variations of spoken dementia, potentially impacting the effectiveness and robustness of the proposed approach. Despite this, we identify key characteristics from the literature and show LLMs and our distilled model's ability to reduce dementia-like features. Our current evaluation also relies on the choice of adversaries given current detection capabilities and does not provide formal guarantees. We attend to this issue by considering several adversaries including traditional and neural classifiers in static and adaptive settings and show the effectiveness of our obfuscation strategy.
In our work, we focus on sentence-level obfuscation and we do not account for intra-sentence dependencies and coherence issues. Future research could explore incorporating such dependencies to enhance obfuscation effectiveness and minimize attribute leakage risk.


%While our primary focus is on this understudied attribute, we believe that our approach and framework can be applied to other attributes as well, such as age, emotion, authorship and gender. Additionally, our PEFT approach allows for the easy sharing of adapter weights for each attribute, depending on the specific use case.

%However, due to the difficulty of accessing dementia datasets, our work relies on only two datasets with the same task which restricts the generalizability of our findings. The data may not fully capture the diverse characteristics and variations of spoken dementia, potentially impacting the effectiveness and robustness of the proposed approach. Nevertheless, we identify key characteristics from the literature and show that LLMs and our distilled model were able to reduce dementia-like features. Our current evaluation also relies on the choice of adversaries given current detection capabilities and does not provide formal guarantees. We attend to this issue by considering several adversaries including traditional and neural classifiers in static and adaptive settings and show the effectiveness of our obfuscation strategy. In our work, we decided to focus on sentence-level obfuscation and we do not account for intra-sentence dependencies that exist within a document. Our approach does not account for repetition or lack of coherence between sentences. Future work can explore how incorporating such dependencies and relationships could further improve the effectiveness of dementia obfuscation and reduce the potential for attribute leakage. 
%\textcolor{red}{A question that might come up, is why we focus only on the dementia attribute? WHat about authorship, gender, emotion, age or other attributes? Is the technique specific only to obfuscate dementia? In which cases is that useful? Do we need other techniques to work orthogonally to this if we want to obfuscate several sensitive attributes?}

%Finally, to achieve the best possible performance, our training strategy updates all of the model's weight during training. This practice is quite computationally expensive and it would be beneficial to explore more efficient training methods similar to prompt and prefix tuning and evaluate the resource usage/performance trade-off.


==> Sections/evalResults_submitted.tex <==
\section{Evaluation Results}
\label{sec:evalResults}

\subsection{Overall Performance and Comparison}\label{sec:evalSetup_overall}
In this section, we aim to answer EQ1 and EQ2 (see Section~\ref{subsec:evalQuestions}).
We compare several baselines (\textit{Pegasus}) and SOTA (\textit{DP} and \textit{ParChoice}) models with our best performing LLM (Mistral) used with zero-shot (ZS), few-shot (FS) and knowledge-based instructions (KB), and with our knowledge distillation approach from Mistral with LoRA adaptation (\systemName{}). Note that a more comprehensive evaluation of LLM performance is presented in Section~\ref{subsec:llmEval}. 

The systems are evaluated for privacy against both our static and adaptive adversary and for utility (semantic preservation). We also indicate the size of each model when relevant as one of our main objectives is to distill knowledge from large language models, into a smaller model. Lastly, we also evaluate the above on both the ADR and the ADRo datasets. Evaluating on ADRo allows us to examine the effects of leveraging automated speech recognition to derive transcriptions for the adversary and the defense mechanisms and is a more challenging scenario compared to the manually transcribed samples of ADR. We summarize the results in Table~\ref{tab:overall-results}.

%\textcolor{red}{Why is it important to show performance on ADReSSo? In what settings this might be useful or more realistic compared to ADReSS?} T

\begin{table*}[!ht]
\centering
\caption{Privacy/utility performance for ADReSS and ADReSSo datasets by different systems. This table presents the F1 score against static (S) and adaptive (A) dementia classifiers, and the average F1 score (Avg F1) across all classifiers. It also depicts semantic preservation (Sem.). We mark our best systems in bold. $\downarrow$ illustrates the defense mechanism aims to decrease that value, and $\uparrow$ to increase it.}
\label{tab:overall-results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lll|cc|cc|>{\columncolor{blue!35}}c|>{\columncolor{blue!35}}c|cc|cc|>{\columncolor{blue!35}}c|>{\columncolor{blue!35}}c}
\toprule

\multirow{3}{*}{\textbf{Type}} &               \multirow{3}{*}{\textbf{Systems}}       &           \multirow{3}{*}{\textbf{\# Params}}           & \multicolumn{6}{c|}{\textbf{ADReSS}}  & \multicolumn{6}{c}{\textbf{ADReSSo}}    \\
\cmidrule(lr){4-9} \cmidrule(lr){10-15}
              &               &             & \multicolumn{2}{c|}{\textbf{BERT\downarrow}} & \multicolumn{2}{c|}{\textbf{SVM\downarrow}} & {\cellcolor{white}}\multirow{2}{*}{\textbf{Avg F1\downarrow}} & {\cellcolor{white}}\multirow{2}{*}{\textbf{Sem.\uparrow}}  & \multicolumn{2}{c|}{\textbf{BERT\downarrow}} & \multicolumn{2}{c|}{\textbf{SVM\downarrow}} & {\cellcolor{white}}\multirow{2}{*}{\textbf{Avg F1\downarrow}} & {\cellcolor{white}}\multirow{2}{*}{\textbf{Sem.\uparrow}}  \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
                  &                      &                      & \textbf{S} & \textbf{A} & \textbf{S} & \textbf{A} & {\cellcolor{white}} \textbf{}  & {\cellcolor{white}} \textbf{} & \textbf{S} & \textbf{A} & \textbf{S} & \textbf{A} & {\cellcolor{white}} \textbf{} & {\cellcolor{white}} \textbf{} \\
\midrule
      Original            & -             & -                    & 0.65        & 0.65          & 0.65        & 0.65          & 0.65 & 1.0 & 0.66       & 0.66         & 0.63       & 0.63         & 0.65 & 1.0            \\
\midrule
    Baselines              & Pegasus              & 568M                 & 0.52       & 0.58         & 0.60       & 0.59         & 0.57 & \textbf{0.85} & 0.5        & 0.57         & 0.58       & 0.58         & 0.56 & \textbf{0.81}       \\
                  & DP$_{T = 1.5}$     & 568M                 & 0.51       & 0.6          & 0.59       & 0.56         & 0.57 & 0.84 & 0.47       & 0.63         & 0.58       & 0.61         & 0.57 & 0.77       \\
                  \cmidrule(lr){2-15}
                  & Parchoice$_{Random}$ & -                   & 0.62        & 0.62          & 0.6         & 0.58          & 0.61 & 0.80 & 0.6        & 0.64         & 0.63       & 0.63         & 0.63 & 0.76       \\
                  & Parchoice$_{SVM}*$  & -                    & 0.55        & 0.58          & 0.51        & 0.50          & 0.54 & 0.84 & 0.58       & 0.64             & 0.51       & 0.61         & 0.59 & 0.76       \\
                  & Parchoice$_{BERT}*$ & 110M                 & 0.65        & 0.62          & 0.67        & 0.58          & 0.63 & 0.78 & 0.65       &  0.62             & 0.61       &  0.6            & 0.62 & 0.74   \\
\midrule
LLMs-based (Ours) & Mistral ZS       & 7B                   & 0.35       & 0.57         & 0.57       & 0.48         & 0.49 & 0.72 & 0.43       & \textbf{0.51}         & 0.57       & 0.61         & 0.53 & 0.64       \\
                  & Mistral FS       & 7B                   & \textbf{0.18}       & 0.5          & 0.55       & 0.51         & 0.43 & 0.62 & \textbf{0.25}       & 0.54         & \textbf{0.31}       & 0.56         & \textbf{0.42} & 0.28       \\
                  & Mistral KB       & 7B                   & 0.31       & 0.63         & 0.55       & 0.57         & 0.52 & 0.78 & 0.36       & 0.58         & 0.52       & 0.58         & 0.51 & 0.67       \\
\cmidrule(lr){2-15}
                  & \systemName{} & 140M (884k adapter) & 0.37       & 0.55         & 0.49       & 0.58         & 0.50 & \textbf{0.85} & 0.4        & 0.58         & 0.5        & \textbf{0.57}         & 0.51 & 0.74       \\
\bottomrule
\footnotesize{$*$ Classifier-dependent}
\end{tabular}%
}
\end{table*}




\vspace{5pt}\noindent\textbf{Automatic Privacy and Utility Analysis of Results.} Compared to Pegasus, DP and all ParChoice versions,  our LLM approaches and \systemName{} achieve better privacy performance on average and on both datasets. In particular, compared to the best version of ParChoice (ParChoice$_{SVM}$), \systemName{} achieves 1.3x better privacy performance or a further 5.7\% decrease in F1-score on the ADR dataset and a more impressive 2.2x improvement in privacy performance or a further 11.2\% decrease in F1-score on ADRo.

%As expected BertTopic obfuscates dementia well on ADR as it only retains abstract topics from sentences. Both the static and adaptive adversary suffered between 41.5\% and 46.1\% decrease in their detection accuracy compared to non-obfuscated (original) sentences on the ADR dataset. Surprisingly, this privacy performance was not transferred to the ADRo dataset where our approaches performed significantly better. A possible reason for this is that there are inherent errors in speech transcriptions which force the ADRo--trained adversarial models to learn more basic representations, such as topics. Importantly, BertTopic also exhibits a non-practical 66\%--70\% decrease in semantic preservation in both datasets. For this reason we discard it as a non-solution from the rest of the analysis.


Importantly we also observe that ParChoice's privacy performance suffers with the ADRo dataset as it cannot deal with speech-to-text errors well, while our approaches exhibit more consistent performance. It's worth noting though that ParChoice$_{SVM}$ does very well in the case the adversary also uses an SVM attack model as we observe a 23.1\% drop in F1-score on the ADR dataset.  However, this is not very realistic, as it assumes the adaptive adversary (with knowledge of the defense mechanism) will use the same model Parchoice was trained against. This is a main limitation of ParChoice as its most performing version is classifier dependent and does \emph{less} well if the adversary does not use the model the defense is using. To better illustrate this, we consider the worst-case scenario for the defense, i.e. when the adversary makes all the best choices of models and datasets to use. In this case, the worst case scenario for ParChoice$_{SVM}$ is against an adaptive BERT adversary on the ADRo dataset where it achieves a lackluster 3.0\% F1-score drop. Comparatively, \systemName{}'s worst-case scenario is against an adaptive SVM adversary on the ADRo dataset. In this case, our system still achieves a 9.5\% F1-score drop which is at least 3x better compared to ParChoice$_{SVM}$'s worst-case performance.

Another important observation from these experiments is that \systemName{} retains the privacy and semantic preservation performance of the zero-shot (ZS) and knowledge-based (KB) LLMs, and their generalizability across adversarial scenarios and datasets. In addition it only requires fine-tuning $\mathcal{O}(10^5)$  parameters compared to fully fine-tuning the $\mathcal{O}(10^{8})$ student model.
%$\mathcal{O}(10^8)$, $\mathcal{O}(10^8)$ and $\mathcal{O}(10^9)$ required in Pegasus, ParChoice and Mistral respectively.

Lastly, all models achieve good semantic preservation with values close to 0.7 and above. Pegasus achieves the best values according to our utility metric although the differences are very subtle---our human evaluators ranked our systems better than Pegasus.  Notably, all of the systems exhibit a semantics drop on the ADRo dataset. This is because there are inherent errors from the automatic speech recognition used to derive the ADRo transcriptions that make high-quality paraphrasing more challenging. The Mistral few-shot LLM (Mistral FS) exhibits the worse utility performance. This is further examined in Section~\ref{subsec:llmEval}, and the paraphrasing quality and users' perception of the semantics of the best systems are analyzed in more depth in Section~\ref{subsec:llmEval} and Section~\ref{subsec:qualSemanticsEval}. 

%Pegasus and DP also achieved unstable performance on privacy: between 3\% (DP, SVM, Adaptive, ADReSSo) to 28.7\% (DP, BERT, static, ADDReSSo) decrease in ASR. However, Pegasus as a SOTA paraphrasing approach achieved very good semantic preservation with decrease between 15\% and 19\% on ADDReSS and ADDReSSo respectively. Note that values of \textcolor{red}{XX} are considered good values for semantic preservation~\cite{}.

%ParChoice, as our chosen SOTA attribute obfuscator achieved similar obfuscation performance with the non-obfuscating paraphrasing model Pegasus: between -3.1\% (Parchoice$_{BERT}$, SVM, Static, ADDReSS) and 23.1\% (Parchoice$_{SVM}$, SVM, Adaptive, ADDReSS). We also observe in a lot of cases,  that the SVM adversary is very robust but more so against Parchoice$_{BERT}$ paraphrases. The best privacy guarantees among ParChoice configurations can be offered by Parchoice$_{SVM}$ (23.1\%) when the adversary \textcolor{red}{Why SVM adaptive on ADReSSo does so much better though?} uses an SVM model. However this is not very realistic, as it assumes the adaptive adversary (with knowledge of the defense mechanism) will use the same model Parchoice was trained against. This is the main limitation of ParChoice as its most performing Parchoice$_{SVM}$ and Parchoice$_{BERT}$ versions are classifier dependent and do less well if the adversary does not use the model the defense is using. ParChoice$_{Random}$ which is not classifier dependent does not do well in privacy (0.0\% to 10.8\% ASR decrease). 

%In terms of our approaches, we first observe that the few-shot (FS) LLM achieved impressive drop in ASR, even outperforming BertTopic in several cases. However, similarly with BertTopic is not useful as it exhibits a significant drop in semantics. This is because...

%The ZS and KB LLMs on the other hand achieve more consistent privacy performance and in most cases significantly better compared with ParChoice. ParChoice can only do better when it is trained explicitly against the model the adversary will use which as explained is not a realistic assumption. The consistency can be attributed to the fact that LLMs are classifier independent and thus generalize better. They both also significantly improved over the FS approach's semantic preservation and are comparable with ParChoice (our human evaluation showed that user's perceive LLM outputs to preserve semantics better compared to ParChoice---see Section~\ref{subsec:humanEval}).

%Most importantly, our improved knowledge-distilled model, retains the privacy and semantic preservation performance of the ZS and KB LLMs, and their generalizability across adversarial scenarios. It clearly is a more effective obfuscator compared to ParChoice in all but one scenario where ParChoice trains an SVM model and the adversary also uses SVM in an adaptive setting, and only on the ADReSS dataset.   
%It also enjoys similar performance in semantic preservation compared to ParChoice. In addition it only requires training $\mathcal{O}(10^5)$  parameters compared to $\mathcal{O}(10^8)$, $\mathcal{O}(10^8)$ and $\mathcal{O}(10^9)$ required in Pegasus, ParChoice and Mistral respectively.


\vspace{5pt}\noindent\textbf{Impact on Key Differentiator in Dementia Detection.} 
To assess the privacy performance of different systems, we analyzed their impact on 10 key linguistic features relevant to dementia detection, based on existing literature. \cite{fraser2016linguistic,emmery2018style,Kempler2008LANGUAGEAD}. These features capture the disfluency (interjections), and the lexical complexity (number of syllables per word) but also markers for memory loss such as higher usage of verbs, pronouns and adverbs to compensate for forgetting a specific noun. To focus on the systems at hand (and not on automated speech recognition effects) we pick ADR for our case study.
On Table~\ref{tab:ad_feats} we report our evaluation results for the five best-performing systems: ParChoice\(_{SVM}\), Pegasus, DP, Mistral\(_{KB}\), and \systemName{}. We see that both Mistral\(_{KB}\), and \systemName{} achieve significant reductions in the proportion of interjections ($-96.83\%$ and $-94.52\%$) and adverbs ($-35.67\%$ and $-57.74\%$). They also show relatively important improvements in increasing the proportion of nouns ($+8.53\%$ and $+6.16\%$) and for Mistral$_{KB}$, the mean syllables per word ($+6.39\%$). Pegasus and DP also reduce interjections, adverbs, and generic nouns and increase total nouns but to a much lesser extent. They stand out in reducing the verbs/nouns ($-18.87\%$, $-16.4\%$) and adverbs/nouns ratio ($-48.85\%$, $-49.31\%$) and increasing modals ($+23.54\%$, $+23.91\%$). They, however, decrease the proportion of mean syllables and increase generic verbs, emphasising dementia-like features. These results can be explained by the summarising tendencies of the models. ParChoice$_{SVM}$ shows notable reductions in generic verbs ($-29.90\%$) and nouns ($-21.29\%$) but adds a significant amount of disfluency ($+41.04\%$) and reduces verbs and modals. ParChoice$_{SVM}$'s impact on the other features, albeit positive, is marginal compared to the other systems. This is expected, as Parchoice relies more on singular and targeted typos and substitutions than paraphrasing. 


%We see that both Mistral\(_{KB}\), and \systemName{} achieve significant reductions in the proportion of interjections (-96.83\% and -94.52\%) and adverbs (-35.67\% and -57.74\%). They also show substantial improvements in increasing the proportion of nouns (+8.53\% and +6.16\%) and for Mistral\(_{KB}\), the mean syllables per word (+6.39\%). Pegasus and DP also reduce interjections (-3.12\%,-4.15\%), adverbs (-29.50\%, -27.50\%), and generic nouns (-19.61\%, -7.89\%) and increase total nouns (0.11\%, 1.73\%) but to a much lesser extent. They, however, decrease the proportion of mean syllables (-1.94\%, -1.91\%) and increase generic verbs (+18.47\%, +19.20\%). They are also very good at reducing the verb/nouns (-18.87\%, -16.4\%) and adverbs/nouns ratio (-48.85\%, -49.31\%). These results can be explained by the summarising tendencies of the models.



\begin{table}
\centering
\caption{Effect (in \%) on key dementia characteristics by best systems the ADReSS dataset. Values going in the direction of control-like features are highlighted and we mark in bold the top-2 systems per feature. }
\label{tab:ad_feats}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
 & \textbf{ParChoice$_{SVM}$} & \textbf{Pegasus} & \textbf{DP} & \textbf{Mistral$_{KB}$} & \textbf{\systemName{}} \\
\midrule
\textbf{Prop. Interjections}$\downarrow$ & 41.04 & {\cellcolor{lightgreen}} -3.12 & {\cellcolor{lightgreen}} -4.15 & \bfseries {\cellcolor{lightgreen}} -96.83 & \bfseries {\cellcolor{lightgreen}} -94.52 \\
\textbf{Prop. Adverbs}$\downarrow$ & {\cellcolor{lightgreen}} -15.09 & {\cellcolor{lightgreen}} -27.50 & {\cellcolor{lightgreen}} -29.50 & \bfseries {\cellcolor{lightgreen}} -35.67 & \bfseries {\cellcolor{lightgreen}} -57.74 \\
\textbf{Mean Syllables Per Word}$\uparrow$ & {\cellcolor{lightgreen}} \bfseries 1.90 & -1.94 & -1.91 & \bfseries {\cellcolor{lightgreen}} 6.39 & {\cellcolor{lightgreen}} 0.34 \\
\textbf{Prop. Nouns}$\uparrow$ & {\cellcolor{lightgreen}} 5.54 & {\cellcolor{lightgreen}} 0.11 & {\cellcolor{lightgreen}} 1.73 & \bfseries {\cellcolor{lightgreen}} 8.53 & \bfseries {\cellcolor{lightgreen}} 6.16 \\
\textbf{Prop. Modals}$\uparrow$ & -17.57 & {\cellcolor{lightgreen}} 23.54 & \bfseries {\cellcolor{lightgreen}} 23.91 & {\cellcolor{lightgreen}} 8.11 & \bfseries {\cellcolor{lightgreen}} 23.66 \\
\textbf{Prop. Verbs}$\uparrow$ & -7.44 & {\cellcolor{lightgreen}} 3.70 & \bfseries {\cellcolor{lightgreen}} 3.81 & \bfseries {\cellcolor{lightgreen}} 3.52 & -3.95 \\
\textbf{Ratio Verbs/nouns}$\downarrow$ & {\cellcolor{lightgreen}} -5.48 & \bfseries {\cellcolor{lightgreen}} -18.87 & \bfseries {\cellcolor{lightgreen}} -16.40 & 12.64 & {\cellcolor{lightgreen}} -9.70 \\
\textbf{Ratio Adverbs/nouns}$\downarrow$ & {\cellcolor{lightgreen}} -16.11 & {\cellcolor{lightgreen}} -48.85 & \bfseries {\cellcolor{lightgreen}} -49.31 & {\cellcolor{lightgreen}} -33.19 & \bfseries {\cellcolor{lightgreen}} -60.11 \\
\textbf{Generic. Nouns}$\downarrow$ & \bfseries {\cellcolor{lightgreen}} -21.29 & {\cellcolor{lightgreen}} -19.61 & {\cellcolor{lightgreen}} -7.89 & {\cellcolor{lightgreen}} -14.62 & \bfseries {\cellcolor{lightgreen}} -26.31 \\
\textbf{Generic. Verbs}$\downarrow$ & \bfseries {\cellcolor{lightgreen}} -29.90 & 18.47 & 19.20 & {\cellcolor{lightgreen}} \bfseries -23.74 & {\cellcolor{lightgreen}} -3.88 \\
\bottomrule
\end{tabular} %
}
\end{table}

\vspace{5pt}\noindent\textbf{Summary of Results.} 
Our evaluation shows that:

\vspace{3pt}\noindent$\bullet$ ZS and KB LLMs are better obfuscators compared to the SOTA text paraphrasing model and the SOTA attribute obfuscator.

\vspace{3pt}\noindent$\bullet$ Both the KB LLM and our distilled model consistently perform more meaningful changes across multiple linguistic metrics than the other systems. ParChoice$_{SVM}$ lacks particularly behind and introduces disfluencies.

\vspace{3pt}\noindent$\bullet$ Our distilled model even though it has one order of magnitude less parameters ($\mathcal{O}(10^8)$) compared to the teacher LLMs ($\mathcal{O}(10^9)$), it retains the LLM's performance in obfuscating dementia in text, and in preserving the semantics of the original sentence, it generalizes to different adversarial scenarios and datasets, and it only requires fine-tuning three orders of magnitude less parameters ($\mathcal{O}(10^5)$) compared to full fine-tuning for our specific task.


\subsection{LLMs as Dementia Obfuscators}
\label{subsec:llmEval}
In the above analysis, we used our most effective LLM. To answer EQ3, here we compare different LLM choices. We compare four open-source models \textit{Gemma, Phi3, Mistral and Llama3}. %These were chosen because they are open source and thus allow us to perform the study without sharing our sensitive data with a third-party. 
We perform a number of experiments testing different LLM models' ability to preserve privacy and preserve semantics. We then delve deeper into the generation ability of LLMs and further analyze the changes introduced by the various models when given the more abstract instruction of ``obfuscating dementia'' (zero-shot setting).


\vspace{5pt}\noindent\textbf{Privacy and Utility.}
For each LLM model, we compare three prompt strategies: zero-shot (\textit{ZS}), few-shot (\textit{FS}), and knowledge-based (\textit{KB}). The results are summarized on Table~\ref{tab:llm-performance}. We see that all systems perform particularly well against the static adversaries but have mixed results against the adaptive ones. We observe a general pattern between different prompting strategies. FS achieves the best privacy scores but also the lowest semantics ($\leq$0.61). This is due to the models mimicking the problem when they were given the example sentences (see Table~\ref{tab:hits_miss}), which they all seem to suffer from. On the other hand, the KB setting improves the semantics for all systems but Gemma, for better performance against static adversaries and comparable performance against adaptive adversaries. The KB strategy particularly improves Llama3 semantics (ZS 0.68 $\rightarrow$ KB 0.82). We note that Llama3 in ZS had failed outputs due to censorship (see Table~\ref{tab:hits_miss}) and observe that it was no longer the case with KB. Both Gemma and Phi3 models have good privacy scores overall despite their relative sizes but are still slightly worse than Mistral and LLama3 models and fall behind in semantics preservation. In ZS setting, Mistral achieves the best overall privacy/utility performance with 0.72 semantics and drops the F1-scores of 46\%, 12\% for the BERT adversary and 12\%, 26\% for the SVM static and adaptive adversaries respectively. In the KB setting, Llama3 achieves the best privacy/utility tradeoff and the highest semantics score (0.82). In our comparison experiments (Section~\ref{sec:evalSetup_overall}) we used Mistral as our representative LLM as it had a more consistent performance across the different prompting strategies.

\begin{table}[!htbp]
\centering
\caption{Privacy and Utility Performance of various LLMs.  This table presents the F1 score against static and adaptive dementia classifiers as well are semantic preservation score. The best results for each column are marked in bold.}
\label{tab:llm-performance}
\resizebox{\columnwidth}{!}{%
 \begin{tabular}{lc|cc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\# Params}} & \multicolumn{2}{c|}{\textbf{BERT$\downarrow$}} & \multicolumn{2}{c|}{\textbf{SVM$\downarrow$}} & \multirow{2}{*}{\textbf{Semantics$\uparrow$}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
 &  & \textbf{Static}  & \textbf{Adaptive}  & \textbf{Static}  & \textbf{Adaptive} & \\
\midrule
Original           & -        & 0.65 & 0.65       & 0.65 & 0.65      & 1.0       \\
\midrule
Gemma ZS       & 2B       & 0.46 & 0.59       & 0.62 & 0.63      & 0.75      \\
Gemma FS       & 2B       & 0.22 & 0.6        & 0.39 & \textbf{0.37}      & 0.61      \\
Gemma KB       & 2B       & 0.28 & \textbf{0.49}       & 0.51 & 0.6       & 0.73      \\
\midrule
Phi3 ZS            & 3.8B     & 0.38 & 0.55       & 0.55 & 0.61      & 0.64      \\
Phi3 FS            & 3.8B     & 0.19 & 0.53       & \textbf{0.18} & 0.6       & 0.36      \\
Phi3 KB            & 3.8B     & 0.27 &  0.54          & 0.5  & 0.58      & 0.74      \\
\midrule
Mistral ZS     & 7B       & 0.35 & 0.57       & 0.57 & 0.48      & 0.72      \\
Mistral FS     & 7B       & 0.18 & 0.5        & 0.55 & 0.51      & 0.62      \\
Mistral KB     & 7B       & 0.31 & 0.63       & 0.55 & 0.57      & 0.78      \\
\midrule
Llama3 ZS & 8B       & 0.39 & 0.52       & 0.57 & 0.55      & 0.68      \\
Llama3 FS & 8B       & \textbf{0.17} & 0.53       & 0.37 & 0.49      & 0.57      \\
Llama3 KB & 8B       & 0.37 &  0.54          & 0.48 & 0.55      & \textbf{0.82}      \\
\bottomrule
\end{tabular}%
}
\end{table}


\vspace{5pt}\noindent\textbf{Paraphrasing Quality.} We analyse the differences at the sample level between different LLMs in a zero-shot setting. We add top-performing systems from Section~\ref{sec:evalSetup_overall} for further analysis. Some examples of samples from the LLMs are shown in Appendix~\ref{app:llms_samples}. Results are shown in Table~\ref{tab:llm_quality}. Among LLMs, Gemma and Mistral perform similarly across the metrics, despite their size difference, showing high semantics (0.75) and METEOR scores (0.56, 0.53). They also have high formality scores (0.72, 0.75) and the lowest perplexity scores (71, 97), making them the most machine-like language models. Phi3 falls in-between with lower semantics preservation and diverges the most from the source (low METEOR and Simi$_{Lex}$). Llama3 remains the closest to the source vocabulary in terms of Simi$_{Lex}$ but has low semantics and METEOR scores. It is the most human-like across the LLMs with a formality of 0.56 and perplexity of 382. All LLMS make a higher number of substitutions ($\geq$0.47) than the other systems as well as additions ($\geq$0.13), except for Parchoice$_{SVM}$ (0.19). On the other hand, Parchoice$_{SVM}$ has a significantly lower formality score (0.23) and higher perplexity (1018), which can be explained by the introduction of disfluencies noted in Section~\ref{sec:evalSetup_overall}. Its samples remain the closest to the source material, with no deletions being recorded. All three language model-based Pegasus, DP and \systemName{} perform similarly across metrics and have the highest semantic preservation but have the lowest perplexities and percentage of additions and the highest proportion of deletions. This indicates a tendency to write sentences more concisely. Overall, LLMs exhibit stronger paraphrasing abilities, often leading to more drastic changes compared to other systems.


\begin{table}[h]
\centering
\caption{Quality Metrics for the zero-shot (ZS) sampling strategy for various LLMs and best-performing systems on the ADReSS dataset. We note S, \% SUB, \% ADD, \% DEL and Simi$_{Lex}$ as semantics, percentages of substitutions, additions, deletions and lexical similarity respectively. }
\label{tab:llm_quality}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{S} & \textbf{Formality} & \textbf{METEOR} & \textbf{\% SUB} & \textbf{\% ADD} & \textbf{\% DEL} & \textbf{Simi$_{Lex}$} & \textbf{Perplexity} \\
\midrule
Gemma       & 0.75               & 0.72               & 0.56            & 0.47                   & 0.13               & 0.12               & 0.65              & 71                 \\
Phi3            & 0.64               & 0.67               & 0.31            & 0.67                   & 0.23               & 0.10               & 0.53              & 180                \\
Mistral     & 0.75               & 0.75               & 0.53            & 0.52                   & 0.23               & 0.10               & 0.63              & 97                 \\
Llama3 & 0.68               & 0.56               & 0.37            & 0.56                   & 0.13               & 0.14               & 0.71              & 382                \\
\midrule
Parchoice$_{SVM}$       & 0.84               & 0.23               & 0.86            & 0.35                   & 0.19               & 0             & 0.79              & 1018                 \\
Pegasus       & 0.85               & 0.8               & 0.63            & 0.35                   & 0.05               & 0.24             & 0.78              & 142               \\
DP$_{T=1.5}$       & 0.84               & 0.8               & 0.61            & 0.36                   & 0.06               & 0.23             & 0.77              & 157              \\
\midrule
\systemName{}       & 0.85               & 0.79               & 0.64            & 0.3                   & 0.06               & 0.21             & 0.76              & 114              \\


\bottomrule
\end{tabular}%
}
\end{table}


\begin{comment}
\begin{table}[h]
\centering
\caption{Quality Metrics for the zero-shot (ZS) sampling strategy on the ADReSS dataset for various LLMs. We note S, \% SUB, \% ADD, \% DEL and Div$_{Lex}$ as semantics, percentages of  substitutions, additions, deletions and lexical diversity respectively. }
\label{tab:llm_quality}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{S} & \textbf{Formality} & \textbf{METEOR} & \textbf{\% SUB} & \textbf{\% ADD} & \textbf{\% DEL} & \textbf{Div$_{Lex}$} & \textbf{Perplexity} \\
\midrule
Gemma       & 0.75               & 0.72               & 0.56            & 0.47                   & 0.13               & 0.12               & 0.65              & 71                 \\
Phi3            & 0.64               & 0.67               & 0.31            & 0.67                   & 0.23               & 0.10               & 0.53              & 180                \\
Mistral     & 0.75               & 0.75               & 0.53            & 0.52                   & 0.23               & 0.10               & 0.63              & 97                 \\
Llama3 & 0.68               & 0.56               & 0.37            & 0.56                   & 0.13               & 0.14               & 0.71              & 382                \\
\bottomrule
\end{tabular}%
}
\end{table}
\end{comment}


\vspace{5pt}\noindent\textbf{LLM Shortcomings.} Table~\ref{tab:hits_miss} presents an overview of failed outputs we encountered with the various LLMs when generating text. These failures range from misunderstanding prompts and refusing to produce potentially offensive content (only observed in Llama3) to contradicting outputs and unrelated tangents. In the case of the few-shot strategy, models often overfit on the given sentences and output texts mimicking their content. There were also instances of instructions not being followed where the model repeats them or simply outputs verbose instead of the correct output. These examples emphasize some of the challenges of using LLMs for automatic data labelling and generation, besides data cleaning and processing. However, these cases made up circa 4\% of the generated outputs (excluding FS) and did not transfer through distillation.




\begin{table}[h!]
\centering
\caption{Examples of failed LLMs outputs.}
\label{tab:hits_miss}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ p{0.28\columnwidth}  | p{0.3\columnwidth} | p{0.6\columnwidth}}
\toprule
\textbf{Type} & \textbf{Input} & \textbf{Output} \\
\midrule
Copying (Few-shot) & what do i see in this picture. & I see a picture with a mother standing in the water and a little girl laughing at her brother taking a cookie from the jar \\
\midrule
Refusal & everything that's going on okay. & I cannot create dementia samples or any other type of content that may be offensive or harmful to individuals with dementia or their caregivers. \\
\midrule
"Hallucination" & and I don't know what the hand means to the mouth. & I understand that the hand is a part of the body that is used for many things, including grasping, pointing, and writing. \\
\midrule
Contradiction & looks like they dried & looks well-hydrated \\
\midrule
Repeating Instructions & and let's see. & Please provide the sentence you'd like me to rewrite, and I'll follow the format to create both dementia and healthy samples. \\
\midrule
"Idem" & and he's about to hand her a cookie. & Keep it the same, no need to replace as the given healthy sentence is already clear \\
\bottomrule
\end{tabular}%
}
\end{table}


%\vspace{3pt}\noindent\textbf{Ability to follow synthetic dataset and refusal count.}

\subsection{\systemName{} Ablation Study}
To better understand how different \systemName{} design decisions affect obfuscation and semantics preservation (EQ4 and EQ5), we design several versions of our obfuscator model. Table~\ref{tab:distill_params} summarizes our results. 

%we design several versions of our obfuscator (a) \textit{BART\_ParaNMT}, \textit{BART\_Mistral\_KB}, and \textit{BART\_Mistral\_KB\_LORA}. \textit{BART\_ParaNMT} is a version which does not use LLMs. It finetunes BART on the ParaNMT dataset, a dataset of more than 50 million English-English sentential paraphrase pairs. This serves as a basic version aiming to train BART to generate high-quality and diverse sentences without any control over the target attribute. \textit{BART\_Mistral\_KB} uses our knowledge-based instructions (KB) to generate sentences with Mistral. These sentences are then used to fully fine-tune BART. Lastly, \textit{BART\_Mistral\_KB\_LORA} is our final version of the model which avoids full fine-tuning using LoRA adaptation.

\vspace{5pt}\noindent\textbf{Base model.} First, we investigate the impact of the smaller model architecture on the overall performance and implement our system with BART and T5 base models. T5$_{KB}$ performs well in adaptive settings (0.53 SVM, 0.56 BERT) but has lower performance for static adversaries and semantics than BART$_{KB}$. T5 is also nearly double the size (220M) of our BART model (140M), adding unnecessary overhead for little gains. 

\vspace{5pt}\noindent\textbf{Dataset.} To evaluate the importance and quality of the synthetic dataset, we also train our model on a popular paraphrasing dataset, ParaNMT~\cite{wieting2017paranmt}, and call this system BART$_{ParaNMT}$. We find that BART$_{ParaNMT}$ generally performs worse in terms of privacy compared to other models having little impact on the adversaries and a lower semantic score (0.84). This shows that a typical dataset of paraphrasing pairs is not sufficient to obfuscate dementia. 

\vspace{5pt}\noindent\textbf{Prompt Strategy.} We fully fine--tune our model on the different synthetic datasets generated by Mistral in ZS, FS and KB settings. We note that the effect of the prompting strategies is less apparent through the distillation method than with the LLMs. Surprisingly, the FS has a bigger drop in semantics ($1.0\rightarrow0.8$) w.r.t ZS and KB ($1.0\rightarrow0.87$), while achieving the best privacy score on the static adversaries (0.29 BERT, 0.42 SVM). BART$_{ZS}$ performs slightly worse than BART$_{KB}$ for the same semantics scores.  We observe that distillation has a soothing effect on the model's performance, thanks to the model's pre--training (both BART and T5). We select BART$_{KB}$ as the best model.

\vspace{5pt}\noindent\textbf{PEFT.} Finally, we compare different PEFT approaches. We observe that BART$_{KB\_IA3}$ has little impact on the obfuscation abilities and naturally preserves the highest semantics, while BART$_{KB\_BOFT}$ has slightly worse results than BART$_{KB\_LoRA}$ with better semantics (0.87 vs 0.85). We retain however BART$_{KB\_LoRA}$ as the best model architecture for \systemName{} as it has the better privacy/utility trade-off.


\begin{table}[h]
\centering
\caption{Influence of model architecture, dataset, prompting strategy and PEFT approaches on the privacy-utility performance of \systemName{} on the ADReSS dataset.}
\label{tab:distill_params}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll|cc|cc|c}
\toprule
\multirow{2}{*}{\textbf{Parameter}}&
\multirow{2}{*}{\textbf{Model}} &
\multicolumn{2}{c|}{\textbf{BERT$\downarrow$}} & \multicolumn{2}{c|}{\textbf{SVM$\downarrow$}} & \multirow{2}{*}{\textbf{Semantics$\uparrow$}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & \textbf{Static} & \textbf{Adaptive} & \textbf{Static} & \textbf{Adaptive} & \\
\midrule
& Original & 0.65 & 0.65 & 0.65 & 0.65 & 1.00 \\
\midrule
\multirow{2}{*}{\textbf{Model}} &BART$_{KB}$ & 0.34 & 0.59 & 0.52 & 0.65 & 0.87 \\
&T5$_{KB}$ & 0.44 & 0.56 & 0.57 & \textbf{0.53} & 0.85 \\ 
\midrule
\multirow{1}{*}{\textbf{Dataset}} & BART$_{ParaNMT}$ & 0.60 & 0.58 & 0.62 & 0.60 & 0.84\\
\midrule
\multirow{3}{*}{\textbf{Prompt}} &
BART$_{ZS}$ & 0.40 & 0.63 & 0.54 & 0.58 & 0.87 \\
& BART$_{FS}$ & \textbf{0.29} & 0.59 & \textbf{0.42} & 0.75 & 0.8 \\
\midrule
\multirow{3}{*}{\textbf{PEFT}} &
BART$_{KB\_IA3}$ & 0.47 & 0.60 & 0.60 & 0.65 & 0.89 \\
& BART$_{KB\_BOFT}$ & 0.40 & 0.56 & 0.54 & 0.58 & \textbf{0.87} \\
& BART$_{KB\_LoRA}$ & 0.37 & \textbf{0.55} & 0.49 & 0.58 & 0.85 \\
\bottomrule
\end{tabular}%
}
\end{table}




\begin{comment}
\begin{table}[h]
\centering
\caption{CTS Ablation}
\label{tab:cts-ablation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|cc|cc|c}
\toprule
\textbf{Dataset} & \textbf{Systems} & \textbf{Static BERT} & \textbf{Adaptive BERT} & \textbf{Static SVM} & \textbf{Adaptive SVM} & \textbf{Semantics} \\
\midrule
\multirow{4}{*}{\centering ADReSS} & Original             & 0.65 & 0.65 & 0.65 & 0.65 & 1.0 \\
                                    \cline{2-7}
                                    & BART\_ParaNMT        & 0.62 & 0.58 & 0.62 & 0.60 & 0.84 \\
                                    & BART\_Mistral\_KB    & 0.34 & 0.59 & 0.52 & 0.66 & 0.87 \\
                                    & BART\_Mistral\_KB\_LORA & 0.37 & 0.55 & 0.49 & 0.58 & 0.85 \\
\midrule
\multirow{3}{*}{\centering ADReSSo} & Original             & 0.62 & 0.62 & 0.65 & 0.65 & 1.0 \\\cline{2-7}
                                     & BART\_Mistral\_ZS    & 0.49 & 0.61 & 0.56 & 0.61 & 87  \\
                                     & BART\_Mistral\_ZS\_LORA & 0.46 & 0.61 & 0.58 & 0.57 & 87  \\
\bottomrule
\end{tabular}%
}
\end{table}

\end{comment}

%\subsubsection{Distillation parameters}

%\vspace{3pt}\noindent\textbf{Impact of architecture}

%\vspace{3pt}\noindent\textbf{Impact of PEFT}


\subsection{Qualitative Semantic Preservation}
\label{subsec:qualSemanticsEval}
Lastly, to answer EQ6 and EQ7, we conduct further analyses on the ability of the best-performing models to preserve semantics.
%\subsubsection{Human Evaluation}
%\label{subsec:humanEval}

\vspace{5pt}\noindent\textbf{Human Evaluation} As mentioned in Section~\ref{sec:evalSetup}, automated semantic similarity metrics do not always align with human judgement. To mitigate this threat to validity we further design an evaluation of semantic preservation with human subjects.
In our study, we select our top five competing systems (ParChoice\(_{SVM}\), Pegasus, DP, Mistral$_{KB}$ and \systemName{}) and ask participants to rate a paraphrase of an original sentence on a 1 to 5 Likert scale. We randomise the questions' order as well as the system’s position within the questions, to mitigate the order bias that might affect how the respondent answers. We recruit 100 participants who are English natives from the UK or US and recruit an additional 60 participants to correct for low-quality respondents (not passing attention checks, not giving meaningful answers, not following instructions)~\cite{douglas2023data}. We split 40 documents into 4 cohorts of 40 participants. Each participant was asked 10 questions. More details on ethical compliance can be found in Appendix~\ref{app:ethics}. %We advertised the survey on Prolific~\cite{prolific}, a platform increasingly used in academic studies as it gives researchers access to a pool of quality participants~\cite{tang2022replication}. Each user is anonymized and accesses the survey online. More details on the ethical compliance can be found in Appendix~\ref{app:ethics}.

The results of our study are summarized in Table~\ref{tab:human_eval}. We observe that Mistral$_{KB}$ archives the highest semantic score (3.86). It is closely followed by \systemName{} with a mean score of 3.75. A paired t-test (with Holm-Bonferroni correction for many comparisons) suggests no significant difference between the two systems. Pegasus and DP are not too far behind, but (statistically) significantly lower. ParChoice$_{SVM}$ has the lowest semantics score of 2.45.   
These results contrast with those of the automatic metrics, Mistral$_{KB}$ having a much higher ranking and ParChoice$_{SVM}$ having a lower score. These results also confirm the shortcomings of the automatic metrics, unable to capture semantics for paraphrases with higher diversity (Mistral$_{KB}$) and/or with small variations (ParChoice$_{SVM}$). Additionally, while the full dataset generated by Mistral$_{KB}$ might have incorrect outputs which might lower the overall semantic score, the survey samples showcased the potential of the LLM on successful outputs.


\begin{comment}
\begin{table}[!h]
\centering
\caption{Mean and standard deviation of human evaluation for different systems. A score of 1 indicates no semantic similarity and 5 identical meaning. The symbols * and $\dagger$ represent systems pairs non significantly different from each other. }
\label{tab:human_eval}
\begin{tabular}{ll}
\toprule
       \textbf{System}        & \textbf{Semantics $\uparrow$}  \\
\midrule
ParChoice$_{SVM}$   & 2.45 ± 0.57     \\
Pegasus             & 3.55 ± 0.46*    \\
DP$_{T=1.5}$       & 3.45 ± 0.47*     \\
Mistral$_{KB}$	     & \textbf{3.86 ± 0.51}$\dagger$    \\
\systemName{}  & 3.75 ± 0.47$\dagger$	      \\
\bottomrule
\end{tabular}
\end{table}
\end{comment}

\begin{table}[!h]
\centering
\caption{Mean and standard deviation of semantic (S) human evaluation for different systems. A score of 1 indicates no semantic similarity and 5 identical meaning. The symbols * and $\dagger$ represent systems pairs non significantly different from each other.}
\label{tab:human_eval}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
& \textbf{ParChoice$_{SVM}$} & \textbf{Pegasus} & \textbf{DP$_{T=1.5}$} & \textbf{Mistral$_{KB}$} & \textbf{\systemName{}} \\
\midrule
\textbf{S $\uparrow$} & 2.45 ± 0.57 & 3.55 ± 0.46* & 3.45 ± 0.47* & \textbf{3.86 ± 0.51}$\dagger$ & 3.75 ± 0.47$\dagger$ \\
\bottomrule
\end{tabular}%
}
\end{table}

\vspace{5pt}\noindent\textbf{Qualitative Sample Comparison} Table~\ref{tab:ad_obf_samples} and Table~\ref{tab:cc_obf_samples} show generated samples for each of the obfuscation approaches. We pick two sentences, one from a control subject and one from a dementia subject, to showcase the structural differences for similar meanings. The AD sample is longer and has a stutter (``the m the mother'') while the control sample uses fewer words. We can see that ParChoice$_{SVM}$ introduces changes in words and typos, consequently decreasing fluency and sense. We note that both Pegasus and \systemName{} rewrite the sample more concisely. On the other hand, ParaNMT paraphrases the text and makes a mistake (``the water was running out of the
water.") or lowers the language level (the mother $\rightarrow$ mom) while Mistral increases the formality level for the AD sample. All systems except ParChoice$_{SVM}$ managed to remove the original disfluencies.

\begin{table}[h]
    \centering
    \caption{Obfuscating a Dementia (AD) sample sentence.}
    \label{tab:ad_obf_samples}
    \begin{tabular}{p{0.21\columnwidth}p{0.65\columnwidth}}
              \toprule
        \textbf{Obfuscation}              & \textbf{Sample} \\
        \midrule
        \textbf{Original AD}              & well in the first place the m the mother forgot to turn off the water and the water's running out the sink. \\
        \midrule
        \textbf{Parchoice$_{\text{SVM}}$} & well in the firstly place the m the mother left to turn off the water and the waters running out the sink. \\
        \textbf{Pegasus}                  & The mother forgot to turn off the water and the water was running out of the sink. \\
        \textbf{DP$_{\text{T=1.5}}$}      & The mother forgot to turn off the water and the sink ran out. \\
        \textbf{ParaNMT}                  & first of all, the mother forgot to turn off the water, and the water was running out of the water. \\
        %\textbf{Mistral$_{ZS}$}               & In the beginning, my mother accidentally left the water running at the sink. \\
        %\textbf{Mistral$_FS$}            & The mother accidentally left the water running in the sink. \\
        \textbf{Mistral$_{KB}$}             & The mother forgetting to turn off the water resultated in it flowing out of the sink. \\
        %Ours$_{ZS}$                & In the first place, the mother forgot to turn off the water and the water is spilling into the sink. \\
        %Ours$_FS$                & The mother forgot to turn off the water and the water is running out the sink  \\
        \textbf{\systemName{}}    &  The mother forgot to turn off the water and the water is flowing out of the sink. \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{table}[h]
    \centering
    \caption{Obfuscating a Control (CC) sample sentence.}
    \label{tab:cc_obf_samples}
    \begin{tabular}{p{0.21\columnwidth}p{0.65\columnwidth}}
    \toprule
        \textbf{Obfuscation}                  & \textbf{Sample} \\
        \midrule
        \textbf{Original CC}         & the mother is uh washing dishes and the water's spilling over on the uh kitchen floor. \\
        \midrule
        \textbf{Parchoice$_{\text{SVM}}$} & the mother is uh washing lookers and the waters spill over on the uh kitchen floor. \\
        \textbf{Pegasus}             & The mother is washing dishes in the kitchen. \\
        \textbf{DP$_{\text{T=1.5}}$} & The mother is washing dishes while the water spills over on the kitchen floor. \\
        \textbf{ParaNMT}             & mom's washing dishes, and there's water all over the kitchen floor. \\
        %\textbf{Mistral$_{ZS}$}     & The mother is washing the dishes, but water is spilling onto the kitchen floor. \\
        %\textbf{Mistral$_{FS}$}     & The mother is washing the dishes, but some water is splashing onto the kitchen floor. \\
        \textbf{Mistral$_{KB}$}     & The mother is washing dishes, but the water is spilling onto the kitchen floor. \\
        %\textbf{Ours$_{ZS}$}      & The mother is washing the dishes, and the water is spilling onto the kitchen floor. \\
        %\textbf{Ours$_{FS}$}      & The mother is washing dishes and the water is spilling onto the kitchen floor  \\
        \textbf{\systemName{}} & The mother is washing dishes and the water is spilling onto the kitchen floor.   \\
        \bottomrule
    \end{tabular}
\end{table}

==> Sections/evalSetup_submitted.tex <==
\section{Evaluation Setup}
\label{sec:evalSetup}

\subsection{Evaluation Questions}\label{subsec:evalQuestions}
We conduct a comprehensive evaluation aiming to answer the following concrete questions: (\textbf{ EQ1}) How effective is our knowledge distillation method through an LLM--generated dataset?;
(\textbf{ EQ2}) How do our proposed obfuscation methods compare to state--of--the--art and baseline approaches?;
(\textbf{ EQ3}) How effective are LLMS in obfuscating dementia and preserving semantics?;
(\textbf{ EQ4}) How do different components of our knowledge distillation method contribute to performance (utility/privacy)?;
(\textbf{ EQ5}) How do obfuscation systems impact key dementia discriminative features (privacy)?;
(\textbf{ EQ7}) How do the generated sentences compare qualitatively with the original sentences?

\begin{comment}
\vspace{3pt}\noindent$\bullet$\textbf{ EQ1.} How effective is our knowledge distillation method through an LLM--generated dataset?

\vspace{3pt}\noindent$\bullet$\textbf{ EQ2.} How do our proposed obfuscation methods compare to state--of--the--art and baseline approaches?

\vspace{3pt}\noindent$\bullet$\textbf{ EQ3.} How effective are LLMS in obfuscating dementia and preserving semantics?

\vspace{3pt}\noindent$\bullet$\textbf{ EQ4.} How do different components of our knowledge distillation method contribute to performance (utility/privacy)?

\vspace{3pt}\noindent$\bullet$\textbf{ EQ5.} How do obfuscation systems impact key dementia discriminative features (privacy)?

\vspace{3pt}\noindent$\bullet$\textbf{ EQ6.} What is users' perception of our methods' ability to preserve semantics (utility) and how does it compare with other methods?

\vspace{3pt}\noindent$\bullet$\textbf{ EQ7.} How do the generated sentences compare qualitatively with the original sentences?
\end{comment}

\subsection{Datasets}
%\vspace{5pt}\noindent\textbf{Dementia Datasets.}  
We use two available datasets which are widely studied in the field of dementia classification: ADReSS~\cite{luz2020alzheimer} and ADReSSo~\cite{luz2021detecting}. The ADReSS (ADR) dataset is a curated subset of the DementiaBank dataset~\cite{becker1994natural}, a collection of 500 recordings from individuals with various stages of dementia. The samples were manually transcribed with dysfluency annotations for the task of the Cookie Theft Picture description. The speakers were selected to be balanced for gender and age, and they split evenly into control (CC) and dementia (AD) groups (54 train and 24 test for each class, a total of 156 samples). In our experiments, we use the provided train/test splits and split the documents on sentence level. We further remove sentences with less than 3 words. We end up with 1179 samples (619 CC $|$ 560 AD) in the training set and 500 (270 CC $|$ 230 AD) in the test and validation sets. The ADReSSo (ADRo) dataset is another subset of DementiaBank designed for detecting dementia from spontaneous speech only, without access to manual transcriptions. The original set consists of 151 train samples (87 CC $|$ 74 AD) and 71 test samples (35 CC $|$ 35 AD). We use the provided segmentation timestamps to isolate segments spoken by the patients and transcribe them using Whisper, a SOTA speech-to-text model~\cite{radford2023robust}. We get 1421 samples in the train set (710 CC $|$ 711 AD) and 644 samples (347 CC $|$ 297 AD) in the test and validation sets. 

\subsection{Adversarial Models}
In evaluating the ability of obfuscators to preserve privacy it is important to consider an adversary in both a static and an adaptive setting. In the former case, the adversary uses available datasets to train the adversarial model. In the second, stronger scenario, the adversary also has knowledge of the defense mechanism.
We implement both a static and adaptive adversary as described below.

\vspace{3pt}\noindent\textbf{Static Adversary.} We finetune a pre-trained BERT-base model with a classifier head as our neural adversary. BERT has been shown to have SOTA performance for various NLP tasks ~\cite{fabien-etal-2020-bertaa,sun-etal-2019-utilizing,bert_age_gender}. We use the base model from\cite{yuan2020disfluencies}\footnote{We evaluate both the base and large versions but pick the base model as it was more robust to obfuscation.} with a learning rate of 1e-6, 10 epochs with early stopping (patience =1 on validation loss), gradient clipping of 1, input length limit of 256 tokens,  and batch size of 8. We also select an SVM as a kernel-based baseline, as presented by ~\cite{luz2020alzheimer} and ~\cite{woszczyk22_interspeech}. We extract a TF-IDF matrix from the corpus and feed it to an SVM with radial-basis-function kernel and $C$ =1.0. The TF-IDF matrix also focuses on different features with learned word frequencies and relative frequencies while BERT looks at the big picture and overall fluency.

\vspace{3pt}\noindent\textbf{Adaptive Adversary.}  We assume the adversary knows which obfuscator is being used, and that they have black-box query access to it. Based on this, we train both SVM and BERT models with the output of the target obfuscation model.

%Topic Modeling (no syntax), Pegasus Paraphrase with T (syntax + semantics), ParChoice (rule-based), Mutant-X, A4NT, Pick most diverse syntax + Best model to reproduce(AESOP-h4?)/ SCPN?

%Our Models: prompt-base syntax BART, syntax-bart with code embeddings.


\subsection{Metrics}
\vspace{3pt}\noindent\textbf{Privacy.} We measure the privacy gain through the drop on the various adversaries' F1-score, for both static and adaptive settings. We refer to the F1-score as the adversary success rate (ASR). We use the F1 metric as it is less sensitive to data imbalance, and shows the model's ability to capture dementia cases and transform dementia samples to control-like ones. 

\vspace{3pt}\noindent\textbf{Utility.} There are currently no available dementia datasets that are labeled for specific tasks such as topic modeling or sentiment analysis. Therefore, for our utility metric, we
focus on semantic preservation. Semantic preservation in natural language is
a powerful primitive that is important for several downstream tasks such as topic modeling, patient and customer complaint analysis, note-taking, etc. 
%To evaluate semantic preservation we conduct (a) comparison with automated metrics, (b) comparison with human subjects, and (c) qualitative comparison of output sentences. 
 We automatically compute the semantic similarity between the original sentence and the output of a selected obfuscation model. We use ParaBART~\cite{huang2021disentangling}, a BART-based model trained to create syntax-invariant semantic embeddings. Common semantic embedding models suffer from poor robustness to different syntax and thus would lower the semantic score between two sentences with different structures even if the meaning is the same. ParaBART on the other has been shown to be more robust to such changes. 

Automated metrics, however, do not always align with human judgment. To mitigate this threat to the validity of our evaluation, we also design a targeted study with human subjects. Our study is designed to measure users' perception of the ability of different text paraphrasing models to preserve the semantics of original sentences. Our study was reviewed and received approval from our institution's research ethics review board. Lastly, we further provide a qualitative analysis of the paraphrase quality of different systems: we select representative sentences from our dataset and compare them with the output of competing systems.

%The benefit of automated metrics is that they allow us to scale our analysis to several systems and parameters as opposed to human subject studies and qualitative analyses which are conducted on a sentence by sentence case. In addition human studies are cumbersome to design and conduct, time-consuming and costly. 

\vspace{3pt}\noindent\textbf{Quality and Diversity Metrics.} To better understand the effect of different systems we measure the quality and diversity of the generated samples by computing the formality score, METEOR score ( a common metric that measures word matches, synonyms, and word order.)~\cite{lavie2009meteor}, lexical similarity (Simi$_{Lex}$) measured by the word-level Levensthein distance between sets of unique words, perplexity and the percentage of substitutions (\% SUB), additions (\% ADD) and deletions (\% DEL) between the source and generated samples. We compute an automatically generated formality score of a sentence by using a RoBERTa model from the Hugging Face library\footnote{https://huggingface.co/s-nlp/roberta-base-formality-ranker} trained on the formality-style transfer dataset GYAFC ~\cite{rao-tetreault-2018-dear} and online formality corpus~\cite{pavlick2016empirical}. Given that neural text generation creates samples with word distribution that are distinct from human-written text, we also investigate the perplexity (PPL) of our generated samples. A high perplexity is commonly associated with human text but is also a sign of low fluency. 
%We use this metric to monitor fluency loss or gain between different approaches. 
We compute the perplexity by computing the exponentiated average negative log-likelihood of a pre-trained GPT2 model using the \textit{lmppl} library\footnote{https://github.com/asahi417/lmppl}. 



%Apart from our utility and privacy metrics, text generation methods need to also demonstrate ability to generate high quality and diverse sentences.  We measure the quality and diversity of the samples generated by different LLMs leveraging established text metrics such as the length of the newly generated samples, \textit{lexical diversity}, the \textit{formality} score, and \textit{perplexity} (described above). The formality score is computed as described in Section~\ref{sec:motivation}. In addition, we also measure the percentage of refusals (no paraphrase returned by the LLM) as this is an important limitation of LLM usage.

\subsection{Obfuscation Models}

%In our evaluation, we use several models to compare our obfuscation approach (\systemName{}). Since \systemName{} is akin to a paraphrasing approach, we pick a state--of--the--art paraphrasing model as baseline. Finally, we compare our system against state--of--the--art obfuscation models which we tailor for dementia.
%We use several models in our evaluation. In particular, we compare our obfuscation approach (CTS) with a baseline model, a state--of--the--art paraphrasing model, and a heuristic-based model. For our baseline, we chose a popular topic modeling model. This is because our goal is to preserve semantics while obfuscating dementia. Topic modeling is designed to extract semantically meaningful topics as a collection of sets of words where each set can semantically describe the same topic. Therefore it could potentially be enough to preserve high semantics in a sentence while obfuscating dementia with little effort. It is also important to compare CTS with a state--of--the--art paraphrasing model. This is because CTS employs a paraphrasing approach and therefore we want to explore whether the best paraphrasing model can be enough to obfuscate dementia while preserving semantics. Since paraphrasing is designed to improve a sentence's clarity it should at least be able to preserve semantics well. Because paraphrasing on its own is not designed for obfuscating attributes, lastly, we want to compare with a state--of--the--art obfuscation model. 
%Below we describe each of the baseline, paraphrasing, and heuristic-based models we implemented.

    %\vspace{3pt}\noindent\textbf{BERTopic (Baseline).} Our topic modeling baseline aims to remove syntax information from the text and represent each sentence using the top-n words from the given topic. To this end, we train a BERTopic model~\cite{grootendorst2022bertopic} on the DementiaBank training set. BERTopic is a variant of the BERT model specifically designed for topic modeling tasks. Using the trained BERTopic model, we replace each sentence with top 5 words of the detected topic. We do this for both test sets of ADReSS and ADReSSo. This baseline helps us understand the impact of removing syntax and preserving only the main information (topic) of the sentence.

    \vspace{3pt}\noindent\textbf{Pegasus (Paraphrasing Model).} We compare our approach to the state-of-the-art paraphrasing model. We employ a Pegasus model~\cite{zhang2020pegasus} fine-tuned to perform paraphrasing on the input text. Pegasus is a transformer-based model that has shown impressive performance in generating high-quality text and paraphrases. It was pre-trained on a large corpus with the task of retrieving important masked sentences and later fine-tuned on paraphrase pairs.
    
    \vspace{3pt}\noindent\textbf{DP (Differential Privacy Obfuscation Model).} 
    Following work by~\cite{mattern2022limits}, we re-implement a text generation model that performs obfuscation by sampling with higher temperatures. We select Pegasus as our language model and do our best to improve on~\cite{mattern2022limits} ---our version is bigger and trained on a larger dataset than their model, to maximize the quality of the generated samples. We also experiment with various temperature values (see Appendix~\ref{app:dp}).

    \vspace{3pt}\noindent\textbf{ParChoice (Heuristics-based Obfuscation Model).} ParChoice~\cite{grondahl2020effective} is a rule-based obfuscation model that has been shown to have good obfuscation abilities while preserving semantics and utility. The model performs a series of modifications such as changing writing voice, contractions, typos, synonyms, etc. It also performs paraphrase selection via a surrogate profiler for style transfer and filter-generated sentences for fluency and grammatical correctness. This approach outperforms simpler rule-based approaches, but also complex models like A4NT~\cite{shetty2018a4nt} and MutantX~\cite{mahmood2019girl} for both obfuscation and semantic retainment.  We use the code made available by the authors and run ParChoice in ``Random'' settings as well as with an SVM and BERT surrogates trained on ADR samples that guide the obfuscation toward a control-like style.

    \vspace{3pt}\noindent\textbf{LLMs (Ours)} We investigate top-performing LLMs for different size brackets in their ability to perform dementia obfuscation.  Due to the sensitive nature of the data, we only use open-sourced models that can be run locally. As ChatGPT and other OpenAI models access and process input data, we omit them in this study. We select Gemma 2B~\cite{team2024gemma}, Phi3 (3B parameters)~\cite{abdin2024phi}, Mistral 7B~\cite{jiang2023mistral} and LLama3 8B~\cite{Llama3is11:online}. We pick Mistral as our best system to train \systemName{} and present all three prompt settings in the summary Table~\ref{tab:overall-results}. We ran each model via the Ollama python library~\footnote{https://github.com/ollama/ollama-python}.
    
\vspace{3pt}\noindent\textbf{\systemName{} (Ours)} We implement our model using the pre-trained \textit{BART-base} model from the Huggingface library\footnote{https://huggingface.co/facebook/bart-base}. We implement and train the core of our system with LoRA (r=16, alpha = 32) on the KB dataset: \systemName{}, and our ablation models: BART$_{KB}$ (full fine-tuning), T5$_{KB}$ (T5 model\footnote{https://huggingface.co/google-t5/t5-base}), BART$_{ParaNMT}$ (trained on paraphrasing dataset ParaNMT~\cite{wieting2017paranmt}), as well as BART$_{KB\_BOFT}$ and BART$_{KB\_IA3}$ for different PEFT techniques: IA3 and BOFT. Intrinsically-Aligned Adapters (IA3) is an adapter technique that injects a small number of trainable parameters (64.5K) into the model. Bottleneck Output-Fusion Transformers (BOFT) introduce a bottleneck layer (138K) to compress and then expand the intermediate representations, to focus on relevant features. We use the paper's default parameters for both.
We finetune our models on the synthetic paraphrase pairs for a maximum of 3 epochs and use early stopping (patience = 10 on validation loss), with a batch size of 8 and a learning rate of 1e-4. At inference time, we sample with the number of beams set to 4 and a maximum length of 256.

==> Sections/exploration.tex <==






\begin{table}[htbp]
\centering
\caption{Comparison of Dementia (AD) and Control (CC) Samples from different Large-Language-Models (LLMs).}
\label{tab:samples}
\begin{tabular}{lp{0.3\columnwidth}p{0.3\columnwidth}}
\toprule
\textbf{System}          & \textbf{Sample AD}                                                      & \textbf{Sample CC}                                                                                      \\ \midrule
\textbf{Original}                  & and uh they're each busy at at uh something.                               & and there's a tree out there somewhere that you can see part of the trunk and part of the foliage.     \\ \midrule
\textbf{Gemma}                & and they were each busy at something.                                      & There is a large tree standing in the distance that you can see some of its branches and leaves.       \\ \midrule
\textbf{Phi3}                      & They are all occupied with their respective tasks.                         & and there's a tree outside where we can catch a glimpse of its trunk and leaves.                        \\ \midrule
\textbf{Mistral}              & And they're all occupied with their own tasks.                             & Outside, you can see a tree with some of its trunk and leaves visible.                                 \\ \midrule
\textbf{LLama3}         & and each person is occupied with their own activity.                        & you can see part of the trunk and some leaves on that tree.                                               \\ \bottomrule
\end{tabular}
\end{table}





==> Sections/introduction_submitted.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[!h]
\centering
\includegraphics[width=0.85\columnwidth]{Figures/Overall_sys/overall_sys.pdf}
\Description{Graph of the AD-GUARD framework. An LLM is used to generate a synthetic dataset of source-obfuscated sentence pairs for a smaller model to train on. The model is trained with PEFT. A source text with a dementia attribute goes through the framework which returns an obfuscated text. An adversary cannot detect dementia but the text can still be used for a downstream task.} 
\caption{Overall structure of \systemName{}. \systemName{} takes as an input a sentence with a potential dementia attribute and generates an obfuscated paraphrase.}
\label{fig:overall_sys}
\end{figure}

Speech is a prevalent human-computer interaction modality and there are strong business incentives for collecting and processing speech data. The size of the Voice Recognition and Speech processing global market amounted to \$12 billion in 2022 and is expected to grow to \$34 billion by 2028.~\cite{mordorintelligenceVoiceRecognition}. The voice assistant market alone is worth \$2.5 billion in 2023 and popular solutions such as Google Home and Amazon Alexa are being used by hundreds of millions of smart speaker users~\cite{statistaSpeakers}. Finance and Telecom companies increasingly rely on speech-to-text APIs and speech analytics to process calls for feedback, categorize queries, and check for compliance with regulations. The healthcare sector is the next biggest use case for speech-to-text as it can speed up note-taking and search and also analyse prevalent topics of worry and patient feedback~\cite{nhschoices}.
%alleviating the strain on the workforce and reducing waiting times for enquiries, and also analyzing prevalent topics of worry and patient feedback~\cite{}. 
Moreover, in this work, we found (see Section~\ref{sec:motivation}) that about 20\% of the most popular Android apps request permission to record audio out of which more than 79\% use APIs to process speech. Transcribing speech allows one to use natural language processing techniques to understand the semantics of the natural language. For example, \textit{Google Keep}~\cite{googleGoogleKeep} is a productivity app with more than 2 billion installations that allows users to take notes using their voice; \textit{Voice Recorder Audio Sound MP3}~\cite{googleVoiceRecorder} and \textit{Otter: Transcribe Voice Notes~\cite{googleOtterTranscribe}} have been installed more than 8 million and 1 million times respectively and produce live and offline voice transcriptions. 

\vspace{3pt}\noindent\textbf{Dementia can be inferred from speech transcripts.} 
Dementia, a degenerative neurological disorder, has become a pervasive global health concern with the ageing population. It affects individuals' cognitive abilities, memory, and overall functioning, and its cases are expected to triple by 2050~\cite{nichols2022estimation}. Disfluencies, mistakes, and signs of cognitive challenge are even more apparent in speech than they are in written text. Key discriminative features were found in speech transcripts and when aggregated, they can be important indicators of Alzheimer's Disease (AD). Recent works on the automatic detection of dementia, yielded promising results~\cite{yuan2020disfluencies,syed2021automated,zolnoori2023adscreen}. These, however, can also be exploited to extract sensitive medical information from transcribed speech. Personal information related to medical conditions is very sensitive and must be kept secret: employers can use it to discriminate against employees or applicants, banks can use it to associate loan applicants with higher risk scores, advertisers can use it to target users, etc. While user attribute leakage has been studied before~\cite{schler2006effects,sarawgi2011gender, emmery2018style, shetty2018a4nt}, little has been done against leakage of medical-related attributes from transcribed speech, such as dementia. 

This is worrisome and it might come in conflict with privacy regulations. For example, GDPR~\cite{gdpr} is an EU regulation that protects the processing of sensitive data. It defines sensitive data as personal data subject to several processing conditions including biometric data and health-related data~\cite{gdprSensitiveData}. GDPR also has \textit{data minimization} as one of its core data protection principles. According to data minimization, data processors must ensure that the data they process are adequate, relevant, and ``\textit{limited to what is necessary}''. Similarly,  
CPRA~\cite{cpra} (California Privacy Rights Act) which took effect in January 2023 and is an amended version of the CCPA (California Consumer Privacy Act) also stipulates that data processors should not process data beyond what ``\textit{reasonably necessary and proportionate to achieve the purposes for which the personal information was collected or processed}''. Therefore, there is a need for solutions that allow understanding of natural language from speech without allowing dementia inference.

%% PRIOR DEFENSE APPROACHES AND LIMITATIONS %%
%koppel2002automatically,abbasi2008writeprints,nguyen2013old
\vspace{3pt}\noindent\textbf{Prior approaches.} 
Several works already exist aiming to either obfuscate sensitive attributes or identity~\cite{koppel2002automatically,abbasi2008writeprints,nguyen2013old,shetty2018a4nt,xu2019privacy, emmery2018style, mahmood2019girl, weggenmann2022dp, mattern2022limits}. Some follow a style-transfer approach to target gender, sentiment, age, and other attributes~\cite{shetty2018a4nt, emmery2018style, mahmood2019girl,xu2019privacy}. These \textbf{(a)} are limited by their dependence on the availability of training data for the specific attributes and \textbf{(b)} they require 
training a model for each new attribute and their obfuscation is hence classifier dependent. 
Medical datasets of conversations and written text for conditions such as dementia are hard to collect and access. Unlike existing style transfer datasets, parallel corpora between patients and control individuals are not available. This limitation calls for methods that can learn to perform obfuscation even in the absence of training data for the target attribute. 
Others have used differential privacy which can provide provable guarantees~\cite{weggenmann2022dp, mattern2022limits}. However, these suffer from poor semantic reconstruction. Furthermore, it is difficult to interpret the privacy metric's ($\epsilon$) value when applied to words in a sentence or a document. More importantly, none of the prior works have been applied to obfuscating sensitive medical attributes such as dementia.

\ignore{
Existing attribute and identity obfuscation approaches are inadequate. 
We can group prior relevant work broadly into three categories: (i) Authorship and attribute obfuscation in text~\cite{koppel2002automatically,abbasi2008writeprints,nguyen2013old,shetty2018a4nt}; (ii) style transfer approaches ~\cite{ shetty2018a4nt, emmery2018style, mahmood2019girl}; and (iii) differential-privacy-based approaches~\cite{weggenmann2022dp, mattern2022limits}. 
We can group prior relevant obfuscation work broadly into two categories:
(i) style-transfer approaches~\cite{shetty2018a4nt, emmery2018style, mahmood2019girl}; and (ii) differential-privacy-based approaches~\cite{weggenmann2022dp, mattern2022limits}.

Obfuscation in text and style transfer have been shown to be effective when applied to gender, sentiment, age, and other attributes, but  (a) they are limited by their dependence on the availability of training data for the specific attributes and (b) they require 
training a model for each new attribute and their obfuscation 
is hence classifier dependent ~\cite{ shetty2018a4nt, emmery2018style, mahmood2019girl}. Medical datasets of conversations and written text for conditions such as dementia are hard to collect and access. Unlike existing style transfer datasets, parallel corpora between patients and control individuals are not available. This limitation calls for methods that can learn to perform obfuscation even in the absence of large training datasets for the target attribute. More importantly, none of these have been applied for obfuscating medical attributes. Prior works using differential privacy have the advantage of providing provable guarantees. However, prior works~\cite{weggenmann2022dp, mattern2022limits} are concerned with authorship obfuscation and do not attempt to conceal specific attributes. More importantly, they suffer from poor semantic reconstruction as they increase the level of noise to conceal the authorship. Furthermore, it is difficult to interpret the privacy metric's ($\epsilon$) value when applied to words in a sentence or a document. 
}

\vspace{3pt}\noindent\textbf{Our Approach.} Our first key idea is to \textit{leverage the capabilities of large language models (LLMs) to perform zero-shot text generation and paraphrasing tasks}. We investigate several open-source LLMs that can be executed privately and design zero-shot, few-shot and knowledge-based instructions to significantly improve privacy performance compared to prior work. However, LLMs require costly memory and computational power due to their $\mathcal{O}(10^9)$ number of trainable parameters, making them impractical for many applications, and they can suffer from hallucinations and refusals. Our second key idea to overcome the LLM limitations is to perform \textit{teacher-student knowledge distillation from LLMs} in a 2-step process: first, we prompt a teacher LLM model to create a dataset of original and obfuscated sentence pairs. Second, we fine-tune a smaller, more efficient student model on this dataset. Fully fine-tuning the smaller model though, still requires training on $\mathcal{O}(10^8)$ parameters. To further improve on this we use our third key idea to \textit{apply a suitable Parameter-Efficient Fine-Tuning} (PEFT) technique. This involves freezing the student's layers, using matrix decomposition to reduce the number of parameters, and integrating lightweight adapter modules. This way we ensure efficient training and reduce computational overhead. Overall, our approach results in a smaller, efficient student model which we call \systemName{} (Knowledge \textbf{Di}stillation from Large-Language-Models for \textbf{D}ementia \textbf{O}bfuscation in \textbf{T}ranscribed \textbf{S}peech). \systemName{} retains the privacy and utility performance of the teacher LLM while requiring three orders of magnitude less parameters ($\mathcal{O}(10^5)$) for fine-tuning. Compared to a state-of-the-art attribute obfuscator (ParChoice~\cite{grondahl2020effective}), \systemName{} is not classifier dependent, achieves 1.3x and 2.2x better on average privacy performance across static and adaptive adversaries on two datasets, and a 3x improvement in a worst case scenario. Human evaluation shows that both our best LLM approach and \systemName{} achieved significantly better comparable utility performance than ParChoice and other baselines.

%Compared to the state-of-the-art attribute obfuscator ParChoice, \systemName{} is not classifier-dependent, achieving 1.3x to 2.2x better average privacy performance against static and adaptive adversaries across two datasets, and a 3x improvement in worst-case scenarios. Human evaluation shows that both our best LLM approach and \systemName{} provide significantly better utility performance than ParChoice and other baselines.


%We introduce a novel approach to obfuscate dementia in transcribed speech. \textcolor{red}{Describe our approach and main results.} We address \textbf{(a)} and \textbf{(b)} by leveraging the capabilities of large language models (LLMs) to perform zero-shot tasks, while also addressing their resource constraints. LLMs require significant memory and computational power, making them impractical for many applications. To overcome this, we use a two-step process: first, we prompt an LLM to create a dataset of original and obfuscated sentence pairs. Second, we train a smaller, more efficient model on this dataset. We utilise recent advances in fine-tuning and apply Parameter-Efficient Fine-Tuning (PEFT) techniques. These involve freezing early layers, using matrix decomposition to reduce the number of parameters, and integrating lightweight adapter modules. This ensures efficient training and reduces computational overhead. Our approach results in a smaller, efficient model that retains the obfuscation capabilities of the LLM, making it more practical for real-world use. %Unlike existing approaches, our method allows us not to rely on \textbf{(b)}.
%The main challenge is to design a method that is independent of the availability of large dementia datasets. 

\ignore{
Our key insight is to use \hl{pairs of document paraphrases} to finetune an existing language model such that it can perform text generation with the intention of paraphrasing an original \hl{document.}
The model can be trained on a non-dementia dataset and applied directly to the sensitive dataset without further training. However, choosing the base model and the paraphrase pairs is not trivial as they determine the quality and structure of the output sequence. Adding to the challenge, text generation and paraphrasing models often produce sequences with non-standardized form, e.g. with grammatical errors, repetition, and nonsensical sentences.
This is problematic because as our analysis shows (see Section~\ref{sec:motivation}) such sequence characteristics are prevalent in dementia samples.
%In particular, we designed a set of features related to standardized speech encompassing fluency, and conciseness and introduced a new metric for analyzing dementia, formality. We then perform a test between dementia and control samples and found statistically significant differences between them for all dimensions.
To address this, firstly we chose BART~\cite{lewis-etal-2020-bart} as our base language model because it is shown to be more robust to errors and to generate more fluent sentences. 
Secondly, we used the PAR3 dataset~\cite{thai2022exploring}, a large-scale dataset of paragraph-level paraphrases, augmented with disfluencies to finetune the generic model for text paraphrasing. This allows us to train a model on longer sequences than current sentence-level paraphrase models and to steer the language model to removing disfluencies.

Another major challenge in obfuscating dementia is to preserve the semantics of the original sentence.
In Section~\ref{sec:motivation} we show that dementia classification can be very effective 
using lexical features. But perturbing lexical features has a penalty on semantics. However, we also show that syntax alone plays a major role in dementia classification. Perturbing syntax should have a much less important adverse effect on semantics.
%Moreover, syntax is independent of lexical features which are important for semantics.
 We leverage this insight and introduce syntactical diversity, using 
a conditional text generation approach.
%a \hl{prompt-tuning approach}~\cite{} 
We first teach the model to learn to generate text given two sentence pairs and their syntax distance
%first learn syntax distances between standardized sentence pairs 
and then prompt the text generation with a desired syntax control knob during inference.

We implemented the above methods into a novel end-to-end language model called 
\textit{Controlled Text Standardization} (CTS).
We evaluated the obfuscation ability of CTS against our most successful traditional and neural-based dementia classifiers. The adversarial classifiers are trained using real dementia datasets both in a static setting (with no knowledge of the defense mechanism) and a stronger adaptive setting where the adversarial models are trained on the output of CTS. We found that CTS is effective with adversaries  
achieving \textcolor{blue}{low F1 scores of 0.41 and 0.49 in the
best case.
We also found that CTS preserves semantics better than the best obfuscating system with Topic Modeling (0.72 vs 0.38 semantic similarity for CTS and BERTopic respectively) at comparable
obfuscation performance (mean of F1 scores of 0.39 for both)
and obfuscates better than a SOTA paraphrasing model for
similar semantic preservation values (0.74 SS for DP
with mean F1-scores of 0.54).}
}

\vspace{3pt}\noindent\textbf{Contributions.} Below we list our main contributions: 

\vspace{3pt}\noindent$\bullet$\textit{ New application domain.} We are the first to explore dementia obfuscation in transcribed speech. We hope this inspires further research on cognitive disorder obfuscation in speech.

\vspace{3pt}\noindent$\bullet$\textit{New Understanding.} We are the first to explore and rigorously evaluate the ability of LLMs to obfuscate dementia and preserve semantics. In doing so we have designed task-relevant zero-shot, few-shot and knowledge-based instructions for LLMs.

\vspace{3pt}\noindent$\bullet$\textit{Novel Obfuscation Method.} We have designed a novel method that effectively distills knowledge from LLMs for dementia obfuscation in a parameter-efficient manner.

\vspace{3pt}\noindent$\bullet$\textit{ Rigorous empirical evaluation and findings.} We perform a systematic and rigorous evaluation of LLMs and our knowledge distillation method across both utility and privacy metrics and through ablation and human studies. We find that LLMs are better obfuscators compared to other competing approaches but have a very large number of trainable parameters ($\mathcal{O}(10^{9})$), and sometimes fail to follow instructions. Our novel \systemName{} method shows that we can learn to obfuscate similarly to LLMs while we only need to partially fine-tune a smaller model ($\mathcal{O}(10^{9})$) on three orders of magnitude less parameters ($\mathcal{O}(10^{5})$) compared to full fine-tuning.

%\vspace{3pt}\noindent$\bullet$\textcolor{blue}{\textit{ New insights.} Unlike previous studies on dementia features, we investigate a new set in view of spoken dementia obfuscation. Specifically, we select indicators relevant to standardization such as fluency, conciseness, and formality, and show significant differences between the two classes.}

%\vspace{3pt}\noindent$\bullet$\textit{ New approach.} We introduce an approach through text standardization that can be applied to low-resource datasets without specialized training which is suitable for obfuscating highly sensitive attributes with low dataset availability.

%\vspace{3pt}\noindent$\bullet$\textit{ New paraphrasing model.} We propose a novel obfuscation language model that can be applied to low-resource datasets. Unlike existing models, our model performs syntactically diverse and standardized sentence paraphrase generation which allows it to obfuscate dementia and preserve semantics.

\vspace{5pt}\noindent\textbf{Ethical Considerations.} In our work, we make use of available upon-request datasets ADReSS and ADReSSo from the TalkBank archive~\cite{macwhinney2004talkbank}, containing recordings and transcripts of conversations with dementia and control patients. Datasets submitted to the TalkBank conform to IRB practices i.e. they are anonymized and do not contain identifiable information. Our human subject study is approved from our institution's Research Ethics review board. Details of our study design are provided in Appendix~\ref{app:ethics}.

==> Sections/method_submitted.tex <==
\section{Dementia Obfuscation in Text}

\begin{figure*}[!h]
\centering
\includegraphics[width=0.9\textwidth]{Figures/Method/detailed_sys.pdf}
\Description{Two sequential blocks showing that an LLM is prompted to generate an obfuscated sentence for each sentence in the set. This dataset goes through processing and is used as input to the second block, model fine-tuning. The figure shows a frozen pre-trained language model fine-tuned with LoRA layers.}
\caption{The two steps of \systemName{}: 1) the creation of a synthetic obfuscated dataset and 2) finetuning a smaller pre-trained language model (PLM) on this dataset with LoRA and a reconstruction loss $L_{CE}$ (cross-entropy). The weights of the PLM are frozen and only matrices A, and B are finetuned. At inference time, the PLM weights are combined with the learned matrices and the model performs obfuscation on input sentences.}
\label{fig:detailed_sys}
\end{figure*}

In this work, we present an approach that takes advantage of the knowledge and rich representations of large-language models (LLMs) to perform dementia obfuscation in text. However, LLMs come with limitations and constraints, the most important one being their size and their operational overhead. Indeed, they require a large amount of resources to both hold them in memory and perform inference in a reasonable time. To tackle this issue, we perform knowledge distillation by prompting an LLM to perform obfuscation (stage I) and recording the [\textit{original}, \textit{obfuscated}] pair to train a smaller and more efficient model on a synthetic dataset (stage II). We further enhance the training efficiency and modularity of our approach fine-tuning our model through a Parameter-Efficient Fine-Tuning (PEFT) method. We describe the different stages of (shown in Figure~\ref{fig:detailed_sys}.) of our methodology in the sections below.

%\subsection{LLMS for AD obfuscation}




\subsection{Knowledge Distillation}
LLMs have important limitations that might render their application to certain settings challenging. One main limitation is their sheer size. For instance, Gemini Ultra by Google has 1.75 trillion parameters ($\mathcal{O}(10^{12})$)~\cite{team2024gemma}. Such models are very computationally expensive and time-consuming to train, with only very few institutions globally having the computational ability and resources to do so. While pre-trained versions exist, some of these are released at the discretion of large institutions, and some are hidden behind paywalls or otherwise kept closed-source requiring sharing of potentially sensitive input data with the model provider. Another limitation of LLMs is that they sometimes fail or refuse to follow instructions. In the first case, this results in an effect coined as hallucination, and in the latter case the model does not return a response.

%\textcolor{red}{can we do a back of the envelope calculation of model size or memory required to train given number of params and a given HW? This could be a contribution we make be choosing LoRA and could be evaluated at the end comparing the HW (GPU cycles), memory requirements, and storage requirements for LLM vs ours.}

Our key insight to overcome those limitations while taking advantage of the powerful nature of LLM in text generation is to \textit{distill knowledge from
from large language models into a smaller model that is easier to train, store and share, and generates more stable output}.

\vspace{3pt}\noindent\textbf{Teacher-student model.} There are several methods to reduce a large model's size. Model compression can be achieved through \textit{quantisation}~\cite{team2024gemma} and \textit{model pruning}\cite{mehta2024openelm,Llama3is11:online}. %For example Gemini Nano~\cite{team2024gemma} is distilled from Gemini Ultra to offer a version with ($\mathcal{O}(10^{9})$) parameters. Similarly Meta's  lightweight version of their LLM, Llama3 8B and Apple's on-device OpenELM~\cite{mehta2024openelm} also have $\mathcal{O}(10^{9})$. Gemini Nano is trivially derived by quantising (4-bit) the bigger Gemini model. 
Such methods, however, aim primarily to reduce the size of the final model. It has been reported that pruning can only be applied for introducing limited sparsity in order to maintain the model accuracy, while quantisation is a lossy process and therefore results in accuracy loss, whether it is used in isolation or in tandem with model pruning techniques~\cite{schaefer2023hardware}. In our work, we leverage knowledge distillation introduced by Hinton et al.~\cite{hinton2015distilling}, where we transfer knowledge from a large, complex model (teacher) to a smaller, more efficient one (student). Specifically, we perform sequence-level knowledge distillation~\cite{kim2016sequence} by generating a synthetic dataset using the larger model's outputs. This approach is more efficient than approximating the teacher's internal states due to the LLMs' size. By distilling the knowledge already learned by the larger model into the smaller one, we create a model that is computationally lighter while retaining much of the performance of the original model. This approach avoids sacrificing the accuracy or complexity of the resulting model, in favor of a bias toward examples specific to our downstream task (fine-tuning).

%\vspace{3pt}\noindent\textbf{Teacher Model} 
Our method is illustrated in Figure~\ref{fig:detailed_sys}. In the first stage, we use an LLM as a teacher model to generate [\textit{original}, \textit{obfuscated}] sentence pairs to create a synthetic dataset to, in stage 2, teach a smaller pre-trained language model (PLM).
Our student model implementation is based on a pre-trained BART model~\cite{lewis-etal-2020-bart}, which is built as a classical Auto-Encoder Transformer. We chose BART due to its good performance and generation quality. Thanks to its denoising pre-training task, BART is more robust to input noise and generates fluent sentences. This is desirable because dementia sentences are less formal and other paraphrasing models tend to produce sentences in non-standardized form. The model is fine-tuned on the synthetic dataset through supervised fine-tuning with cross entropy-loss. Note that BART can easily be replaced in this process with another sequence--to--sequence model. 
%In our evaluation (Section~\ref{sec:evalResults}) we demonstrate the effect of the student model choice.


%\subsection{Data Labeling \& Prompting Strategies}

\vspace{3pt}\noindent\textbf{Data Labeling \& Prompting Strategies.} 
%Our approach embodies a stage where a synthetic dataset is generated using instruction-based LLMs.  
A key step of our approach is synthetic data generation by prompting instruction-based LLMs and relies on the quality of instructions provided to the selected LLM. We follow and compare several strategies to achieve good-quality outputs. Specifically, we prompt an instruction-based LLM to generate an obfuscation candidate for every sentence in our dataset. We use three different prompting strategies as shown in Figure~\ref{fig:prompt_strats}: \textit{zero-shot}, \textit{few-shot}, and \textit{knowledge-based}. To all prompts, we add safeguard instructions to force the model to follow the prompt as closely as possible and avoid rejections or noisy answers.  
In the zero-shot setting, we ask the model to obfuscate a dementia sentence. In the few-shot setting, the model is given 10 examples of dementia and control sentences. Finally, in the knowledge-based prompt, we incorporate knowledge from previous works and dementia detection studies. These have identified that dementia patients tend to be more wordy, and vague, use simpler vocabulary and display highly disfluent speech~\cite{fraser2016linguistic, lancashire2009vocabulary, le2011longitudinal, becker1994natural}.
Based on this we construct an instruction for the LLM asking it to clarify a given sentence. Moreover, in our instruction, we do not mention dementia. This strategy is employed to circumvent the censorship showcased by some LLMs when sensitive topics are mentioned. In the optic of ensuring 'alignment' (a term designating the capacity of a model to follow given ethical and legal guidelines) and reducing risks linked to chatbot usage, companies such as OpenAI, Meta or Google implement various safety measures. These can include experts red teaming and evaluating the safety of prompts~\cite{meta:online, OpenAIRe94:online} and filtering data used for pre-training or post-generation moderation~\cite{openai_mod:online,team2024gemma,abdin2024phi,touvron2023llama}. 
%These policies are put in place to prevent harmful content such as hate speech or promote illegal activities. 
Reportedly, ChatGPT and Llama2 models have shown high levels of censorship (on topics related to politics, gambling or ``killing'' time)~\cite{reuter2023m,Llama3is11:online,Ididntth65:online}, often misinterpreting a benign prompt as unsafe (see examples in table~\ref{tab:hits_miss}). After generation, samples are cleaned from the template to obtain the obfuscated sentence.   

 

\begin{figure}[!h]
\centering
\includegraphics[width=\columnwidth]{Figures/Method/prompts_4.pdf}
\Description{Three bubbles with the text prompt used to query the LLMs: zero-shot, few-shot, knowledge-guided}
\caption{Instructions for zero-shot, few-shot and knowledge-based prompting strategies. We omit few-shot examples for the sake of space.}
\label{fig:prompt_strats}
\end{figure}

\subsection{Parameter-Efficient Fine-Tuning}
As mentioned, we fine-tune our student model using the synthetic dataset. However, we do not perform full fine-tuning but instead employ a Parameter-Efficient Fine-Tuning (PEFT) technique. PEFT is a new paradigm that involves optimizing pre-trained language models for specific tasks by fine-tuning only a small subset of their parameters~\cite{hu2021lora, liu2021p, lester2021power}. Through PEFT we aim to retain the majority of the student model's pre-trained knowledge, making it resource-efficient and faster than full model fine-tuning. Also, by focusing on fewer trainable parameters, we further reduce the risk of overfitting and maintain the model's overall performance.

More specifically we fine-tune our student model using Low-Rank Adaptation (LoRA)~\cite{hu2021lora}, a state-of-the-art PEFT technique. With LoRA, we inject trainable low-rank matrices into each layer of the Transformer architecture, allowing only these matrices to be fine-tuned while the rest of the model remains frozen. Therefore, we can drastically reduce the number of trainable parameters, making the fine-tuning process efficient and preserving the LLM's core knowledge.

With LoRA, the adaptation of the model is achieved by decomposing the weight updates into low-rank matrices. Specifically, for a given weight matrix $W$ in the transformer model, we introduce two smaller matrices $A$ and $B$ such that:

\[
\Delta W = A \cdot B
\]

where $A \in \mathbb{R}^{d \times r}$ and $B \in \mathbb{R}^{r \times k}$, with $r \ll \min(d, k)$. Here, $d$ and $k$ are the dimensions of the original weight matrix $W$. During fine-tuning, only the parameters in $A$ and $B$ are updated, keeping the original $W$ unchanged. The effective weight matrix $W'$ during adaptation thus becomes:

\[
W' = W + \Delta W = W + A \cdot B
\]

This low-rank decomposition significantly reduces the number of parameters that need to be trained, as the number of parameters in $A$ and $B$ combined is much smaller than in the original $W$.

%During training, only the parameters associated with LoRA Modules are updated.

==> Sections/motivation_submitted.tex <==
\section{Understanding the Risks}
\label{sec:motivation}


%\subsection{Security Threat Analysis}
%\subsection{Understanding the Risks}
%As individuals engage with a wide range of digital platforms, their interactions, and voices are increasingly being transcribed into text for further analysis. 

%To better understand the threats of profiling from transcribed speech we (a) 
%investigate the size, and nature of relevant markets, (b) perform a more detailed analysis on speech and transcription data collection and processing on the most popular smartphone OS ecosystem, and (c) identify alarming examples of mobile apps which process speech. 

%To better understand the threats of profiling from transcribed speech we perform a more detailed analysis of speech and transcription data collection and processing on the most popular smartphone OS ecosystem. 
%Then we define our threat model.

%, and (c) identify alarming examples of mobile apps which process speech. 
\ignore{
\vspace{5pt}\noindent\textbf{Market Overview.} The size of the Voice Recognition and Speech processing markets globally is\ignore{estimated to be around \$12 billion in 2022 and is} expected to grow to 34 billion by 2028~\cite{}. The speech-to-text API market and the speech analytics markets were valued at \$2.32 billion (2021)~\cite{} and \$2.3 billion (2022)~\cite{} respectively. Smart speakers also embody voice assistants (e.g. Amazon Alexa, Google Home etc) which collect and transcribe speech to aid in natural language understanding.  The voice assistant market is worth \$2.5 billion and hundreds of millions of users use smart speakers in their house~\cite{statistaSpeakers}. The top applications sectors were found to be healthcare,  banking, financial services and insurance (BFSI), retail, enterprise, consumer, automotive, and education for voice recognition~\cite{},  and the top use cases for Speech-to-text APIs were contact centres, transcriptions, fraud detection, compliance management, voice search and captioning~\cite{}.

%This is driven by several key players such as Google, Amazon, Microsoft, IBM, and Nuance Communications. 
%These technologies have found applications in diverse sectors, from healthcare and customer service to entertainment and education. The top applications sectors were found to be healthcare,  banking, financial services and insurance (BFSI), retail, enterprise, consumer, automotive, and education for voice recognition~\cite{},  and the top use case for Speech-to-text APIs were contact centers, transcriptions, fraud detection, compliance management, voice search and captioning.~\cite{}. Moreover, Amazon Alexa and Google Home have been leading the voice assistant market which is worth \$2.5 billion. More than \hl{X} million users make use of devices powered by Amazon Alexa and Google Home. As it is evident from the above, there are strong business incentives for collecting and processing speech data for millions of users across the world.

%(Shares of X and X respectively within the 2.5 billion total size)~\cite{} and popularising the use of voice-based interfaces among the population (X spread among US population).

%When surveying companies deploying voice solutions they found that “Customer Service” is the most deployed function (81\%), then “Sales” (52%), followed by “Store Operations” and “Marketing and Advertising ( both 38\%)~\cite{}.
}

%\vspace{5pt}\noindent\textbf{Speech-to-Text in Android apps.} To further quantify the prevalence of speech collection and processing, we conducted an analysis on popular mobile apps. 
\subsection{Speech--to--Text in Mobile Apps}
Existing market studies evidence the prevalence and importance of speech-to-text~\cite{enlyftWatsonSpeech,mordorintelligenceVoiceRecognition,statistaSpeakers,Speechto59:online}.
We further systematically quantify the prevalence of speech collection and processing, through an analysis on popular mobile apps, a popular interface with digital services (more than 5 billion people own a smartphone~\cite{statistaSmartphoneUsers}) and because there are available tools for collecting and analyzing mobile apps.
Our analysis focuses on the Android ecosystem because it has the largest ($>70\%$~\cite{androidMarketshare}) mobile OS market share. We collected the top $200$ free Android apps among $54$ application categories from GooglePlay~\cite{googlePlay}, Android's official application store, using \texttt{google-play-scraper}\footnote{https://github.com/facundoolano/google-play-scraper}. This resulted in $10070$ unique apps. For each app, we collected the Android package (\texttt{.apk} and application metadata such as the application's description, its requested permissions, and the number of installations. 

The first goal of our analysis is to study the prevalence of audio collection. Apps collecting audio could infer or leak sensitive information from speech either on purpose or inadvertently. The latter is possible if third-party libraries embedded in the app decide to take advantage of the legitimately granted permission to access audio and further process the audio to identify sensitive user attributes~\cite{grace2012unsafe}, or if the app is compromised~\cite{samsungKeyboardBug, demissie2020security, felt2011permission, tuncay2016draco}. To measure how many of these apps have the capability of collecting audio data, we search their \texttt{AndroidManifext.xml} files for the presence of the \texttt{RECORD\_AUDIO} permission. Developers use these files to provide important information (such as Android permissions) that the system requires to execute their apps. Alarmingly, we found that 20.3\%/10070 apps request permission. These apps have $128$M of installations on average with the most popular app having 15B installations.

Next, we wanted to further understand which of the
 apps which collect audio, specifically perform speech-to-text processing. To detect this, we wrote a script that looks for the presence of the system \texttt{SpeechRecognizer}~\cite{androidSpeechRecognizer} in the code of the apps. However, speech-to-text can be performed using third-party (3P) libraries as well. Therefore we further manually compile a list of 13 APIs based on market leaders~\cite{Speechto59:online} and popular services that we provided to our script. We supplement this list with the API's and popular libraries' SDK calls when available and keywords that search for functions that relate to speech-to-text (full list in Appendix~\ref{app:android_keywords}). Note, that our list is incomplete therefore our script will only provide a conservative estimate.
After removing apps for which decompilation failed, we were left with $1743$ apps.
We found that $1380$ apps ($79.1\%$) are currently employing speech-to-text. $1306$ ($74.9\%$) use the Android's built-in speech recognition system service \texttt{SpeechRecognizer}, 534 ($30\%$) matched for keywords associated with speech-to-text functions and 82 ($4.7\%$) use an API.
%These results indicate an active effort to transcribe or analyze spoken language. Looking at the category distribution we found that the majority of these apps are in the X categories.

To identify if any apps process speech in violation of users' expectations we investigated how many of the apps that use a speech-to-text API in their code do not explicitly mention it in their public descriptions~\cite{pandita2013whyper}. We randomly picked $50$ out of the $1380$ apps and manually went through their descriptions looking for mentions of speech-to-text or transcription activity. Specifically, we look for direct or implied (e.g. speak and it will repeat after you) mentions of ``speech-to-text'' or synonymous tasks such as transcription, dictation, live translation, captioning, and voice-based control. Alarmingly, we found that $42$ ($84\%$) of these apps do not mention it. After further analysis, we found that $1278/1306$ ($98\%$) use the \texttt{SpeechRecognizer} to enable voice search through Android's \texttt{SearchView} widget. Voice search allows the apps access to unfiltered transcriptions of users' queries~\cite{androidCreateSearch}.  This shows that voice control is a prevalent but not adequately described functionality which is increasingly offered by popular apps. To examine whether violations of user expectations happen not only for voice-controlled but also for other speech-to-text processing tasks, we
 repeated the experiment purposively sampling 50 apps that do not only use \texttt{SpeechRecognizer} (616/1380), therefore speech processing is unlikely to be triggered explicitly by the user. We found that 34/50 (68\%) do not refer to speech-to-text in their descriptions.
 

In summary, we found that (a) an important number of popular apps collect audio, (b) most of them transcribe speech, and (c) the transcription functionalities are rarely described in the apps' public descriptions.

%We noticed that  \texttt{SpeechRecognizer} is often linked to Android's \texttt{SearchView} widget which enables voice search and hence we repeated the experiment but limiting ourselves to the 616 apps that also had either keywords/SDKs or both. We found that only 16 out of 50 (32\%) refer to speech-to-text. In our analysis, we observe that unless speech is the core service or the app's description is very rigorous, the transcription or processing functionalities are often hidden.


\subsection{Preliminaries}
\label{sec:bkgd_nlp}

\vspace{5pt}\noindent\textbf{Text Feature Extraction.} 
To process text with algorithms and models, it must first be transformed into numerical form. Tokenization is the fundamental step, splitting words into sub-entities and mapping them to a index in a vocabulary. The simplest feature representation is the Bag-of-Words, which counts token occurrences in a document. The TFIDF matrix improves on this by scaling token frequency relative to the entire corpus, emphasising rare words (often nouns) with potentially more valuable information. However, these methods ignore grammar and word meaning. More advanced approaches like as Word2Vec\cite{mikolov2013efficient}, Glove\cite{pennington2014glove} or FastText\cite{bojanowski2017enriching} build word embeddings, mapping words into a vector space where similar tokens are close-by. Nevertheless, these embeddings lack context awareness, meaning the same word can have different meanings. Attention-based models like BERT~\cite{Devlin2019BERTPO} provide contextual representations, capturing semantic information for sentence level that can be fed to classification models such as neural networks. Contextual embeddings have been shown to hold powerful representations that can be then used for downstream tasks such as sentiment and semantic analysis. Structural information such as Part-of-Speech (POS) tagging and Constituency Parsing can also be extracted. POS tagging assigns grammatical tags to words, indicating their functions within sentences. Constituency parsing creates a syntax tree representing the hierarchical structure of sentences, which can be abstracted into grammar production rules defining permissible word arrangements. Both POS tags and syntax structure are valuable for tasks like attribute or authorship classification, Machine Translation, or Named Entity Recognition.

\vspace{5pt}\noindent\textbf{Language Models.} A language model (LM) is a probabilistic model of a natural language. The model learns a conditional probability distribution $P(w)$ of the next word/token given the sequence of size $n$ of previous tokens. We can write the conditioned distribution as $P(w_{t_{n}}|w_{t_0},w_{t_1},...,w_{t_n-1})$.
Modern LMs, including Large Language Models (LLMs) like ChatGPT\footnote{https://chatgpt.com/} or Llama3\footnote{https://llama.meta.com/Llama3/}, are based on the Transformer architecture~\cite{vaswani2017attention} and predict text in an autoregressive manner (each predicted token depends on the previous ones). The Transformer consists of layers of self-attention mechanisms and feedforward neural networks. Self-attention helps encode the input contextually and capture long-range dependencies within a sentence, while cross-attention between encoded inputs and previous tokens aids in predicting the next token. The model then generates probabilities for each word in the vocabulary using a linear and Softmax layer, at each step. Current LLMs are typically decoder-only models~\cite{brown2020language,abdin2024phi,team2024gemma}, using prompted text as input without cross-attention. 

Recent LMs are pre-trained on large corpora to predict or reconstruct masked sentences and words, learning the language's semantics and patterns in an unsupervised manner. These pre-trained models can then be used to extract meaningful representations useful for downstream tasks such as classification or measuring semantic similarity. The models can also be fine-tuned on specific tasks using smaller, labelled datasets, adapting them for tasks like question-answering or classification. However, with the advance of LLMs, carefully crafted prompts can achieve similar results without fine-tuning, as seen with models like GPT3~\cite{brown2020language}, InstructGPT~\cite{ouyang2022training} and FLAN models~\cite{chung2024scaling}. These models, trained on instructions and human feedback (Reinforcement learning from human feedback), can perform tasks such as paraphrasing, text simplification, or style transfer in zero-shot and few-shot scenarios.


%\vspace{5pt}\noindent\textbf{Knowledge Distillation} 
%Knowledge or Model distillation involves transferring knowledge from a large, complex model to a smaller, more efficient one. This process often involves fine-tuning a smaller model on a dataset generated by the larger model. By distilling the knowledge learned by the large model into the smaller one, it's possible to create models that are computationally lighter while retaining much of the performance.

\vspace{5pt}\noindent\textbf{Dementia Classification.} Dementia is a condition that progressively deteriorates one's cognitive capabilities, affecting their ability to retain and recall information, reason and communicate. Alzheimer's disease (AD) is the most common form of dementia, accounting for approximately 60-80\% of cases. Early detection is key to preventing and providing care for patients with dementia. To this end, several studies investigated differences between a control group and patients with Alzheimer's and found significant changes in syntactical and acoustic indicators~\cite{fraser2016linguistic}. Other found differences in syntactical and lexical features~\cite{le2011longitudinal, lancashire2009vocabulary}. For example, Le et al.~\cite{le2011longitudinal} perform a longitudinal study of four authors and have found that dementia patients demonstrate \emph{lexical indicators} such as a decline in vocabulary and in the usage of complex words, an increased number of low-specificity nouns and verbs, but also \emph{syntactical markers} such as lower frequency of nouns and higher frequency of verbs and lower usage of the passive form.
Recently, machine learning algorithms have been successfully applied for automatic dementia detection from speech (audio) and speech transcripts (text), presenting a cheaper, more efficient, and non-intrusive diagnosis method for patients. 
Garcia et al~\cite{de2020artificial} found that features extracted from the transcripts were often the most indicative of dementia. 
Others used a combination of linguistic and acoustic features, including \emph{pause} and \emph{disfluency} markers.
For example, Yuan et al.~\cite{yuan2020disfluencies} incorporated disfluency tags and silences in the transcript and achieved 89.6\% detection accuracy on the ADReSS \cite{luz2020alzheimer} dataset.

%These approaches have also allowed researchers to look at the most discriminative features in text and in speech for a given model~\cite{de2020artificial}. It was found that features extracted from the transcripts were often the most indicative of dementia. 

%Challenges such as ADReSS \cite{luz2020alzheimer} and ADReSSo \cite{luz2021detecting} accelerated work in the domain. The initial challenge, ADReSS, was designed to offer a standardized and balanced dataset for research to test and develop detection and Mini-Mental State Examination (MMSE) regression methods. The ADReSS set is a curated subset of the DementiaBank dataset. It includes both audio samples and their manual transcriptions and the latter iteration, ADReSSo, provided audio samples only to challenge approaches to focus on spontaneous speech.

%Most successful approaches use a combination of linguistic and acoustic features, including pause and disfluency markers. The best submissions for the ADReSS challenge fine-tuned pre-trained Transformer-based language models such as BERT, Ernie or Roberta. Yuan et al.~\cite{yuan2020disfluencies} incorporated disfluency tags and silences in the transcript and achieved 89.6\% on the test set.  Several of the best-performing submissions to ADReSSo compared multiple automatic transcription models and have found that they can emphasize differences between AD and control patients and when fed to large language models achieve high classification accuracy. 

%However, prior works showed that syntax might be an important discriminative factor in dementia classification~\cite{}.
%To verify this, we also train our classifiers using only syntax TF-IDF features. In particular, we parse each sentence to extract their constituency parse from which we extract only their Part--of--Speech (POS) tags. Then we compute the BoW and TF-IDF matrix for the POS tags of each sentence. The results are shown on Figure~\ref{fig:motivation_clf} (right).
%The success  (0.58 F1 score | 0.66 F1 score) of the syntactically trained classifiers reveals that syntax alone is an important factor in dementia classification. Therefore, \textit{the obfuscation mechanism might be more successful in preserving semantics and obfuscating dementia if it has a larger effect on a sentence's syntax}.

%These are basic models, not used later on.


%We establish a strawman baseline for dementia attribute detection by training models that require little effort and no domain knowledge. In particular, we train an SVM model with TF-IDF features (see Section~\ref{sec:evaluation}) on the ADReSS and DementiaBank datasets and report the mean Matthew's correlation coefficient (MCC) with 10 folds cross-validation, at both sentence and document-level. The MCC is a more accurate representation of the classification performance, especially for imbalanced datasets, with a value of 0 indicating a random classifier. In addition, we also report the mean F1-score and accuracy for further comparison. Figure~\ref{fig:motivation_clf} summarizes our evaluation results: at the sentence-level we achieve F1 and MCC scores of 0.67, and 0.37 respectively for the ADReSS dataset and even higher scores of 0.8 and 0.66 at document-level.

%To further demonstrate the importance of syntax for detecting dementia, we also train a model independently of lexical features. We extract the syntax parse and compute the TF-IDF matrix for Part-of-Speech (POS) tags and train an SVM model. Similarly, we report MCC, F1-score and accuracy. As also evident on Figure~\ref{fig:motivation_clf}, even without semantics the classifiers retain a positive Matthew's correlation with the predictions.  



\begin{comment}
\begin{figure}[!h]
\centering
\includegraphics[width=0.9\columnwidth]{Figures/Motivation/ad_synt_lex_sent_bert.pdf}
\caption{Performance of our baseline dementia classifiers. We report the mean F1-score over 10-folds for BERT trained on raw text (lexical) and part-of-speech tags (syntax), and SVM, LR, and RF models trained on bag-of-words and syntactical features on the ADReSS and DementiaBank datasets.}
\label{fig:motivation_clf}
\vspace{-5pt}
\end{figure}
\end{comment}

%Therefore, the obfuscation mechanism might be
%successful in preserving semantics and obfuscating dementia
%if it has a larger effect on a sentence’s syntax

\subsection{Threat Model}
\label{sec:motivation:threat}
We consider an adversary with access to a target user's transcribed speech. The adversary's goal is to detect whether the target user suffers from dementia. The adversary can operate in two settings: (a) a static setting and (b) an adaptive setting. A static adversary ($\mathcal{A}$) is obfuscation-oblivious and has direct access to the raw text. $\mathcal{A}$ does not have access to any additional information such as age, mental state exam score or audio recordings and has to rely on the text or transcript only. The adversary can gain access to available upon request DementiaBank datasets, blogs or novels, as well as public knowledge of dementia-related stylistic properties. An adaptive adversary ($\mathcal{A}_{Ada}$) is obfuscation-aware. We assume that $\mathcal{A}_{Ada}$ has gained access to samples generated by any applied obfuscation strategy and can leverage these obfuscated samples to adapt and improve their detection capabilities. 

For both scenarios, we consider the adversaries able to implement a kernel-based text classifier (SVM) trained on word token frequencies and a neural network (BERT) able to learn more complex structures and contextual information within a sentence and documents. These were chosen from the ADReSS challenge. The SVM classifier is first described by Luz et al~\cite{luz2020alzheimer} in their paper describing and setting the baselines for the ADReSS INTERSPEECH 2020 challenge. It achieved the best performance across several other classifiers on the test set when using only linguistic features. Our choice of SOTA is the BERT model which won the ADReSS challenge on detecting dementia from text~\cite{yuan2020disfluencies}.

%Our SVM baseline is taken from the paper introducing the ADReSS challenge~\cite{luz2020alzheimer} and our SOTA model from the winning work for that challenge on detecting dementia from text~\cite{yuan2020disfluencies}.

Our defense mechanism aims to perform automatic dementia attribute obfuscation from $\mathcal{A}$ and $\mathcal{A}_{Ada}$ in text while preserving the semantics of the original transcribed speech.

==> Sections/old_distillation.tex <==
\section{Knowledge Distillation}

\subsection{Method}

Explain the general approach.

Synthetic dataset.
PEFT training.

\subsection{Evaluation Setup}


\subsection{\textcolor{blue}{Obfuscation Models}}

In our evaluation, we use several models to compare our obfuscation approach (CTS). We pick a popular topic modeling model as our baseline. Topic modeling is designed to extract semantically meaningful topics as a collection of sets of words where each set can semantically describe the same topic. Therefore it could potentially be enough to preserve high semantics in a sentence while obfuscating dementia with little effort. Since CTS follows a paraphrasing approach, we also compare it with a state--of--the--art paraphrasing model. Finally, we compare our system against state--of--the--art obfuscation models which we tailor for dementia.
%We use several models in our evaluation. In particular, we compare our obfuscation approach (CTS) with a baseline model, a state--of--the--art paraphrasing model, and a heuristic-based model. For our baseline, we chose a popular topic modeling model. This is because our goal is to preserve semantics while obfuscating dementia. Topic modeling is designed to extract semantically meaningful topics as a collection of sets of words where each set can semantically describe the same topic. Therefore it could potentially be enough to preserve high semantics in a sentence while obfuscating dementia with little effort. It is also important to compare CTS with a state--of--the--art paraphrasing model. This is because CTS employs a paraphrasing approach and therefore we want to explore whether the best paraphrasing model can be enough to obfuscate dementia while preserving semantics. Since paraphrasing is designed to improve a sentence's clarity it should at least be able to preserve semantics well. Because paraphrasing on its own is not designed for obfuscating attributes, lastly, we want to compare with a state--of--the--art obfuscation model. 
Below we describe each of the baseline, paraphrasing, and heuristic-based models we implemented.

    \vspace{3pt}\noindent\textbf{BERTopic (Baseline).} Our topic modeling baseline aims to remove syntax information from the text and represent each sentence using the top-n words from the given topic. To this end, we train a BERTopic model~\cite{grootendorst2022bertopic} on the DementiaBank training set. BERTopic is a variant of the BERT model specifically designed for topic modeling tasks. Using the trained BERTopic model, we replace each sentence with the top 3 and top 5 words of the detected topic. We do this for both test sets of DementiaBank and ADReSS since ADReSS is a subset of DementiaBank. This baseline helps us understand the impact of removing syntax and preserving only the main information (topic) of the sentence.
    
    \vspace{3pt}\noindent\textbf{DP Pegasus (DP Obfuscation Model).} 
    Following work by~\cite{mattern2022limits}, we re-implement a text generation model that performs obfuscation by sampling with higher temperatures. We select Pegasus as our language model and do our best to improve it---our version is bigger and trained on a larger dataset than the model in ~\cite{mattern2022limits}, to maximize the quality of the generated samples. We also experiment with various temperature values (see Appendix~\ref{app:dp}).

    \vspace{3pt}\noindent\textbf{ParChoice (Heuristics-based Obfuscation Model).} ParChoice~\cite{grondahl2020effective} (PC) is a rule-based obfuscation model that has been shown to have good obfuscation abilities while preserving semantics and utility. The model performs a series of modifications such as changing writing voice, contractions, typos, synonyms, etc.. It also performs paraphrase selection via a surrogate profiler for style transfer and filter-generated sentences for fluency and grammatical correctness. This approach has been shown to outperform simpler rule-based approaches, but also complex models like A4NT~\cite{shetty2018a4nt} and MutantX~\cite{mahmood2019girl} for both obfuscation and semantic retainment.  We use the code made available by the authors and run ParChoice in ``Random'' settings as well as with an SVM surrogate trained on DB samples that guides the obfuscation toward a control-like style.
    
    \vspace{3pt}\noindent\textbf{CTS (Ours).} We implement our model using
the PyTorch framework and the pre-trained \textit{BART-base} model from the Huggingface library\footnote{https://huggingface.co/facebook/bart-base}. We finetune our model on the annotated paraphrase pairs with the control knob for a maximum of 5 epochs and use early stopping (patience = 10 on validation loss), with a batch size of 8 and a learning rate of 1e-5. At inference time, we sample from the model with the number of beams set to 4 and a maximum length of 256. We implement and train our two core versions of our system: CTS$_{\text{TED}}$ and CTS$_{\text{FK}}$, and our ablation models: CTS (no control code), ParaNMT (no control code \&  no standardization), ParaNMT$_{\text{TED}}$ and ParaNMT$_{\text{FK}}$.

\subsection{Results}

\vspace{5pt}\noindent\textbf{Overall}
\begin{table}[htbp]
\centering
\caption{Comparison of Systems}
\label{tab:comparison}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|cc|cc|c}
\toprule
\textbf{Systems}       & \textbf{CLF} & \textbf{Static} & \textbf{Adaptive} & \textbf{Static} & \textbf{Adaptive} & \textbf{Semantics} \\ \midrule
Original                &              & .65             & .65               & .65             & .65               & 1.0                 \\ \midrule
Parchoice SVM           &              & .55             & .62               & .51             & .50               & .84                 \\ 
Parchoice Random        &              & .62             & .58               & .60             & .58               & .8                  \\ 
ParchoiceBERT           &              & .67             & .62               & .67             & .58               & .78                 \\ \midrule
Mistral\_7B ZS          &              & .35             & .57               & .54             & .48               & 72                  \\ 
Mistral\_7B FS          &              & .18             & .55               & .46             & .51               & 62                  \\ 
Mistral\_7B KB          &              & .39             & ?                 & .51             & ?                 & 72                  \\ \midrule
BART\_Mistral\_ZS       &              & .49             & .61               & .56             & .61               & 87                  \\ 
BART\_Mistral\_ZS\_LORA &              & .46             & .61               & .58             & .57               & 87                  \\ \bottomrule
\end{tabular}%
}
\end{table}
\\
\vspace{5pt}\noindent\textbf{Impact of Paraphrasing Dataset}

See impact of base model on ability to follow synthetic dataset + impact on usual metrics (METEOR, Lexical div, STATIC/AD/SEM)






==> Sections/old_evalResults.tex <==

\begin{table*}[!ht]
\centering
\caption{Privacy/utility performance for ADReSS and ADReSSo datasets by different systems. This table presents the F1 score against static (S) and adaptive (A) dementia classifiers as well are semantic preservation (Semantics). The best results for each column are identified in bold.}
\label{tab:overall-results}
\resizebox{\textwidth}{!}{
\begin{tabular}{lll|cc|cc|c||cc|cc|c}
\toprule

\multirow{3}{*}{\textbf{Type}} &               \multirow{3}{*}{\textbf{Systems}}       &           \multirow{3}{*}{\textbf{\# Params}}           & \multicolumn{5}{c|}{\textbf{ADReSS}}  & \multicolumn{5}{c}{\textbf{ADReSSo}}    \\
\cmidrule(lr){4-8} \cmidrule(lr){9-13}
              &               &             & \multicolumn{2}{c|}{\textbf{BERT\downarrow}} & \multicolumn{2}{c|}{\textbf{SVM\downarrow}} & \multirow{2}{*}{\textbf{Sem.\uparrow}}  & \multicolumn{2}{c|}{\textbf{BERT\downarrow}} & \multicolumn{2}{c|}{\textbf{SVM\downarrow}} & \multirow{2}{*}{\textbf{Sem.\uparrow}}  \\

\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
                  &                      &                      & \textbf{S} & \textbf{A} & \textbf{S} & \textbf{A} &            & \textbf{S} & \textbf{A} & \textbf{S} & \textbf{A} &            \\
\midrule
      Original            & -             & -                    & 0.65        & 0.65          & 0.65        & 0.65          & 1.0        & 0.66       & 0.66         & 0.63       & 0.63         & 1.0            \\
\midrule
Baselines         & BertTopic$_{top5}$     & -                    & 0.35       & \textbf{0.37}         & \textbf{0.38}       & \textbf{0.38}         & 0.34       & 0.66       & 0.57         & 0.45       & 0.57         & 0.3        \\
\cmidrule(lr){2-13}
                  & Pegasus              & 568M                 & 0.52       & 0.58         & 0.60 (\textcolor{red}{$\downarrow7.7\%$})       & 0.59         & \textbf{0.85}       & 0.5        & 0.57         & 0.58 (\textcolor{red}{$\downarrow7.9\%$})      & 0.58 (\textcolor{red}{$\downarrow7.9\%$})        & \textbf{0.81}       \\
                  & DP$_{T = 1.5}$     & 568M                 & 0.51       & 0.60 (\textcolor{red}{$\downarrow7.7\%$})          & 0.59       & 0.56         & 0.84       & 0.47 (\textcolor{green}{$\downarrow28.8\%$})      & 0.63         & 0.58       & 0.61 (\textcolor{red}{$\downarrow3.1\%$})         & 0.77       \\
                  \cmidrule(lr){2-13}
                  & Parchoice$_{Random}$ & -                   & 0.62 (\textcolor{red}{$\downarrow4.6\%$})       & 0.62 (\textcolor{red}{$\downarrow4.6\%$})          & 0.6         & 0.58          & 0.80       & 0.6        & 0.64         & 0.63 (\textcolor{red}{$\downarrow0.0\%$})       & 0.63 (\textcolor{red}{$\downarrow0.0\%$})         & 0.76       \\
                  & Parchoice$_{SVM}*$  & -                    & 0.55        & 0.58 (\textcolor{red}{$\downarrow10.8\%$})         & 0.51        & 0.50          & 0.84       & 0.58       & 0.64 (\textcolor{red}{$\downarrow3.0\%$})           & 0.51       & 0.61         & 0.76       \\
                  & Parchoice$_{BERT}*$ & 110M                 & 0.65        & 0.62          & 0.67 (\textcolor{red}{$\downarrow-3.1\%$})       & 0.58          & 0.78       & 0.65 (\textcolor{red}{$\downarrow1.5\%$})       &  0.62             & 0.61       &  0.6            & 0.74   \\
\midrule
LLMs-based (Ours) & Mistral ZS       & 7B                   & 0.35       & 0.57         & 0.57       & 0.48         & 0.72       & 0.43       & 0.51         & 0.57       & 0.61         & 0.64       \\
                  & Mistral FS       & 7B                   & \textbf{0.18}       & 0.5          & 0.55       & 0.51         & 0.62       & \textbf{0.25}       & 0.54         & \textbf{0.31}       & 0.56         & 0.28       \\
                  & Mistral KB       & 7B                   & 0.31       & 0.63         & 0.55       & 0.57         & 0.78       & 0.36       & 0.58         & 0.52       & 0.58         & 0.67       \\
\cmidrule(lr){2-13}
                  & \systemName{} & 141.18M (884K adapter) & 0.37 (\textcolor{green}{$\downarrow43.1\%$})      & 0.55         & 0.49       & 0.58 (\textcolor{red}{$\downarrow10.8\%$})         & \textbf{0.85}       & 0.4 (\textcolor{green}{$\downarrow39.4\%$})        & 0.58         & 0.5         & 0.57 (\textcolor{red}{$\downarrow9.5\%$})         & 0.74       \\
\bottomrule
\footnotesize{$*$ Classifier-dependent}
\end{tabular}%
}
\end{table*}


==> Sections/old_llms_study.tex <==

\section{LLMS for Dementia Obfuscation in Text}

\subsection{Methodology}

\subsection{Privacy Evaluation Setup}


\vspace{5pt}\noindent\textbf{Dementia Datasets.}  In our work we use two available datasets which are widely studied in the field of dementia classification: ADReSS~\cite{luz2020alzheimer} and ADReSSo. The ADReSS (ADR) dataset is a subset of the DementiaBank dataset~\cite{becker1994natural}, a collection of 500 recordings from individuals with various stages of dementia. The samples were manually transcribed with dysfluency annotations for the task of the Cookie Theft Picture description. The speakers were selected to be balanced for gender and age, and they split evenly into control (CD) and dementia (AD) groups (54 train and 24 test for each class, a total of 156 samples). In our experiments, we use the provided train/test splits. The ADReSSo (ADRo) dataset is another subset of DementiaBank designed for detecting dementia from spontaneous speech only, without access to manual transcriptions. The original set consists of 151 train samples (87 CC $|$ 74 AD) and 71 test samples (35 CC $|$ 35 AD). We use the provided segmentation timestamps to isolate segments spoken by the patients and get 2705 samples in the train set (920 CC $|$ 1026 AD) and 231 samples (74 CC $|$ 87 AD) in the test and validation sets, one per speaker.   

%\subsubsection{Adversarial Models}

\vspace{3pt}\noindent\textbf{Adversarial Models} We finetune a pre-trained BERT-base model with a classifier head as our neural adversary. BERT has been shown to have SOTA performance for various NLP tasks ~\cite{fabien-etal-2020-bertaa,sun-etal-2019-utilizing,bert_age_gender}. We use the base model from\cite{yuan2020disfluencies}\footnote{We evaluate both the base and large versions but pick the base model as it was more robust to obfuscation.} with a learning rate of 1e-6, 10 epochs with early stopping (patience =1 on validation loss), gradient clipping of 1, input length limit of 512 tokens,  and batch size of 8. We also pick an SVM as a kernel-based and naive baseline, as presented by ~\cite{luz2020alzheimer} and ~\cite{woszczyk22_interspeech}. We extract a TF-IDF matrix from the corpus and feed it to an SVM with kernel = radia-basis-function and $C$ =1.0 (selected via 1-fold cross validation). The TF-IDF matrix also focuses on different features than BERT with learned word frequencies and relative frequencies while BERT looks at the big picture and overall fluency. In addition to the \textbf{static adversaries} (trained on raw data),  we also evaluate our systems against \textbf{adaptive adversaries} with knowledge of the defense mechanism. In particular, we train both SVM and BERT--based models with training data which includes the output of the obfuscation model.

%Topic Modeling (no syntax), Pegasus Paraphrase with T (syntax + semantics), ParChoice (rule-based), Mutant-X, A4NT, Pick most diverse syntax + Best model to reproduce(AESOP-h4?)/ SCPN?

%Our Models: prompt-base syntax BART, syntax-bart with code embeddings.


%\subsection{Metrics}
\vspace{3pt}\noindent\textbf{Privacy and Utility Metrics.} We measure the \textbf{privacy} gain through the drop on the various adversaries' F1-score, for both static and adaptive settings. We believe the F1 metric is the most appropriate for our use case as it is less sensitive to data imbalance, and shows us the model's ability to capture dementia cases and transform dementia samples to control-like ones. We measure the \textbf{utility} as semantic preservation, as there are currently no available dementia datasets that are labeled for specific tasks such as topic modeling or sentiment analysis. Semantic preservation in natural language is
a powerful primitive that is important for several downstream tasks such as topic
modeling, patient and customer complaint analysis, note-taking, etc. 
To quantify this we compute the semantic similarity between the original sentence and the output of the obfuscation models.
To compute the semantic similarity we use ParaBART~\cite{huang2021disentangling}, a BART-based model trained to create syntax-invariant semantic embeddings. Common semantic embedding models suffer from poor robustness to different syntax and thus would lower the semantic score between two sentences with different structures even if the meaning is the same. ParaBART on the other has been shown to be more robust to such changes.

\vspace{3pt}\noindent\textbf{Quality and Diversity Metrics} We measure the quality and diversity of the samples generated by different LLMs by computing the length of the newly generated samples, lexical diversity, the formality score, perplexity (described above) and the number of refusals (no paraphrase given by the LLMs). The formality score is computed as described in Section~\ref{sec:motivation}.

\subsection{Results}


\begin{table}[htbp]
\centering
\caption{Privacy Evaluation of LLMS}
\label{tab:comparison}
\resizebox{\columnwidth}{!}{%
 \begin{tabular}{lll|ll|ll|l}
    \toprule
    \textbf{Dataset} & \textbf{System} & \textbf{\# Params} & \textbf{BERT} & \textbf{SVM} & \textbf{Bert\_{Ada}} & \textbf{SVM\_{Ada}} & \textbf{Semantics}  \\
    \midrule
    \multirow{12}{*}{\textbf{ADReSS}}& \textbf{Original} & - & 0.65 & 0.65 & 0.65 & 0.65 & 1.0  \\
    \cmidrule{2-8}
    & Gemma ZS & 2B & 0.46 & 0.62 & 0.76 & 0.73 & 0.75  \\
    & Gemma FS & 2B & 0.22 & 0.39 & 0.79 & 0.8 & 0.61  \\
    & Gemma KB & 2B & 0.28 & 0.51 & 0.72 & 0.68 & 0.73  \\
    \cmidrule{2-8}
    & Phi3 ZS & 3.8B & 0.38 & 0.55 & 0.7 & 0.8 & 0.64  \\
    & Phi3 FS & 3.8B & 0.19 & 0.18 & 0.68 & 0.77 & 0.36  \\
    & Phi3 KB & 3.8B & 0.27 & 0.52 & 0.84 & 0.67 & 0.75  \\
    \cmidrule{2-8}
    & Mistral ZS & 7B & .35 & .57 & .54 & .48 & 0.72  \\
    & Mistral FS & 7B & .18 & .55 & .46 & .51 & 0.62  \\
    & Mistral KB & 7B & .32 & 0.55 & 0.77 & 0.67 & 0.78   \\
    \cmidrule{2-8}
    & LLama3 ZS & 8B & 0.41 & 0.57 & 0.77 & .68 & 0.68  \\
    & LLama3 FS & 8B & 0.18 & 0.37 & 0.68 & 0.55 & 0.57  \\
    & LLama3 KB & 8B & 0.37 & 0.48 & 0.63 & 0.68 & 0.82 \\
    \bottomrule
  \end{tabular}%
  }

\end{table}


We compare our best models and control code, as well as ablation studies CTS and ParaNMT trained with and without control codes, with other models and baselines in terms of privacy and utility and report the results in Figure~\ref{fig:scatter_trade_off} (See Appendix~\ref{app:sent_eval} for exact values). 

Our BERTopic baselines achieve the lowest accuracies (0.38 on ADR \& 0.58 on DB) for our models while losing 40\%-50\% of the original semantics. The results of the topic modeling model confirm that topics are insufficient to detect dementia. On the other hand both the rule-based and paraphrasing models preserved the semantics the best. However, these approaches also perform the worst in terms of obfuscation. In fact, as shown by the perplexity values (PPL) in Figure~\ref{fig:compareTEDPPL}, DP$_{\text{T=2.0}}$ seems to introduce further disfluencies that paraphrase control samples into dementia-like samples due to their more chaotic nature, also indicated by the increased TED. ParChoice (PC) seems to generate less fluent texts but also does not disrupt the syntax much. Our models on the other hand seem to have a standardizing effect with the lowest perplexities and yet disrupt syntax the most. We note, however, that both Pegasus and CTS models lowered the perplexity matching closely to the one of a language model. Both CTS$_{\text{TED}}$ and CTS$_{\text{FK}}$ achieve obfuscation results on a par with BERTopic while having better semantic preservation capabilities (0.36, 0.38 for BERTopic against 0.67 and 0.73 for CTS$_{\text{TED}}$ and CTS$_{\text{FK}}$). We also highlight the positive contribution of the control code indicated by the differences in obfuscation performance for both CTS and ParaNMT models. This approach allowed for uniform syntax constraints for each sentence. This effect was particularly noticeable with BERT, which displayed greater robustness to our models without control codes. Moreover, the dataset choice played an important role in the obfuscation as well, as evidenced by the inferior performance of ParaNMT. Among the standardization metrics, it appears that formality has the most substantial impact, possibly explained by its link with complexity, disfluency, and interjections. We note that the SVM classifier is more robust than the neural approach with BERT. This could be explained by the small dataset size the model was trained on, as neural networks require a larger amount of samples than an SVM. This observation sheds light on the robustness of the current SOTA dementia classifiers. Our best model achieves a 35\% and 25\% (ADR SVM), 51\% and 34\% (ADR BERT), 23\% and 12\% (DB SVM) and 64\% and 27\% (DB BERT) \emph{drop} in static/adaptive adversary success rate compared to non-obfuscated text at sentence level. Both SVM and BERT static/adaptive adversaries drop below random performance on the ADReSS set. This best model achieves semantic similarity with the original text up to 73\% on ADR and  64\% on DB which is comparable with the best prior paraphrasing model, DP$_{\text{T=2.0}}$ which only achieves drops of  17\% and 17\% (ADR SVM), 27\% and 19\% (ADR BERT), 7\% and 7\% (DB SVM), 27\% and 19\% (DB BERT), compared to non-obfuscated text.


\begin{table}[htbp]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
Model           & S_{MNET}    & S_{ParaBART} & Formality          & METEOR             & Lex\_div            & Perplexity         \\
\midrule
Gemma\_2B        & 0.73               & 0.73                & 0.74               & 0.42               & 0.61               & 267.46             \\
Phi3            & 0.74               & 0.75                & 0.85               & 0.41               & 0.60               & 208.92             \\
Mistral\_7B      & 0.76               & 0.78                & 0.80               & 0.48               & 0.65               & 140.37             \\
LLama3\_8B & 0.79               & 0.82                & 0.68               & 0.48               & 0.71               & 469.45             \\
\bottomrule
\end{tabular}%
}
\caption{Quality metrics for KB setting.}
\label{tab:my_label}
\end{table}

\begin{table}[htbp]
\centering
\caption{Comparison of Dementia (AD) and Control (CC) Samples from different LLMs.}
\label{tab:samples}
\begin{tabular}{lp{0.3\columnwidth}p{0.3\columnwidth}}
\toprule
\textbf{System}          & \textbf{Sample AD}                                                      & \textbf{Sample CC}                                                                                      \\ \midrule
\textbf{Original}                  & and uh they're each busy at at uh something.                               & and there's a tree out there somewhere that you can see part of the trunk and part of the foliage.     \\ \midrule
\textbf{Gemma 2B}                 & and they were each busy at something.                                      & There is a large tree standing in the distance that you can see some of its branches and leaves.       \\ \midrule
\textbf{Phi3}                      & They are all occupied with their respective tasks.                         & and there's a tree outside where we can catch a glimpse of its trunk and leaves.                        \\ \midrule
\textbf{Mistral\_7B}              & And they're all occupied with their own tasks.                             & Outside, you can see a tree with some of its trunk and leaves visible.                                 \\ \midrule
\textbf{LLama3\_Instruct}         & and each person is occupied with their own activity.                        & you can see part of the trunk and some leaves on that tree.                                               \\ \bottomrule
\end{tabular}
\end{table}

\vspace{3pt}\noindent\textbf{Dementia and Text Standardization.}
%There have been many features, both linguistic and acoustic, investigated for dementia detection. Features such as lexical complexities, POS tag distribution, grammar rules, and idea densities were all successfully applied to assess the cognitive state of patients and improve the classification of dementia samples. However, 
Motivated by the discriminative power of syntax and disfluencies for dementia detection and how they deviate from control patients, we also investigate features related to how ``standard text'' would look. To this end, we identify and design a set of features relevant to text standardization and use them to perform an analysis on DementiaBank and ADReSS datasets. We divide the features into fluency, formality, and text compression indicators\footnote{We also analyzed figurative speech (metaphors, idioms, hyperboles) but our detection models and ourselves could not reveal any key indicators for none of the samples. The nature of the task might not leave much opportunity for them to occur.}. Our disfluency markers are the proportion of interjection part-of-speech tags (INTJ) and repetitions that can be found in the constituency parse. We compute the parse constituency for both datasets using the Fisher disfluency parser~\cite{jamshid-lou-2020-improving} to catch both markers better. To capture incomplete sentences we compute the mean number of sentences that contain subject and verb tags (S\&V), ones that start with the subject (indicated by the production rule ROOT$\rightarrow$S extracted from the syntax parse), and measure the proportion of nouns without determinants (NP$\rightarrow$NN). We introduce the metric that has not been studied before on dementia, the formality score. We compute an automatically generated formality score of a sentence by using a RoBERTa model from the Hugging Face library\footnote{https://huggingface.co/s-nlp/roberta-base-formality-ranker} trained on the formality-style transfer dataset GYAFC ~\cite{rao-tetreault-2018-dear} and online formality corpus~\cite{pavlick2016empirical}. We also compute complexity, for which we measure the mean number of syllables per word. Finally, we compute the mean sentence length to investigate how concise each sample is. We also report the proportion of adverbs and verbs relative to nouns to capture the replacements of specific nouns by paraphrases. The values are summarized in Table~\ref{tab:standard_anl}.

\begin{table}
\centering
\caption{Mean and standard deviation for standardization metrics on the ADReSS (ADR) and DementiaBank (DB) datasets across both dementia (AD) and control (CC) classes. $\dagger$ denotes statistically significant for $p\leq0.05$.}
\label{tab:standard_anl}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cc|cc}
\toprule
 & \multicolumn{2}{c}{\textbf{ADReSS}} & \multicolumn{2}{c}{\textbf{DementiaBank}} \\
\midrule
 \bfseries Metrics & \textbf{CC} & \textbf{AD} & \textbf{CC} & \textbf{AD} \\
\midrule
\textbf{Formality} & 0.26 (0.11)  $\dagger$ & 0.21 (0.08)  $\dagger$ & 0.28 (0.26) $\dagger$  & 0.18 (0.18) $\dagger$  \\
\textbf{Perplexity} & 897.06 (2818.73) & 1265.22 (9150.72) & 833.1 (5117.78) & 1104.82 (6776.51)) \\
\textbf{Sentence Length} & 9.38 (6.05)  $\dagger$ & 8.31 (5.04)  $\dagger$ & 9.595 (6.836) $\dagger$  & 9.501 (6.577)) $\dagger$  \\
\textbf{Complexity} & 1.24 (0.21)  $\dagger$ & 1.18 (0.21)  $\dagger$ & 1.2 (0.19) & 1.16 (0.184) \\
\textbf{S \& V} & 0.9 (0.3)  $\dagger$ & 0.84 (0.37)  $\dagger$ & 0.91 (0.28) $\dagger$  & 0.88 (0.32) $\dagger$  \\
\textbf{ROOT $\rightarrow$ S} & 0.83 (0.37)  $\dagger$ & 0.7 (0.46)  $\dagger$ & 0.82 (0.38) $\dagger$  & 0.75 (0.43) $\dagger$  \\
\textbf{INTJ count} & 1.36e-2 (5.37e-2)  $\dagger$ & 3.5e-2 (8.97e-2)  $\dagger$ & 2.5e-2 (7e-2) $\dagger$  & 3.08e-2 (7.59e-2) $\dagger$  \\
\textbf{EDIT count} & 7.3e-4 (5.53e-3)  $\dagger$ & 1.75e-3 (8.82e-3)  $\dagger$ & 3.41e-3 (1.1e-2)$\dagger$  & 7.5e-3 (1.72e-2) $\dagger$  \\
\textbf{ADV$/$NOUN} & 0.33 (0.0)  $\dagger$ & 0.46 (0.1)  $\dagger$ & 0.4 (0.27) $\dagger$  & 0.41 (0.3) $\dagger$  \\
\textbf{V$/$NOUN} & 0.59 (0.41) & 0.75 (0.29) & 0.69 (0.41) & 0.72 (0.52) \\
\textbf{PR$/$NOUN} & 0.38 (0.15) & 0.97 (0.42) & 0.63 (0.44) $\dagger$  & 0.74 (0.51) $\dagger$  \\
\textbf{NP$\rightarrow$NN} & 0.14 (0.35)  $\dagger$ & 0.09 (0.29)  $\dagger$ & 0.12 (0.33) $\dagger$  & 0.09 (0.29) $\dagger$  \\
\bottomrule
\end{tabular}%
}
\vspace{-5pt}
\end{table}


As shown in Table~\ref{tab:standard_anl}, most of the features exhibit differences between the two classes. Our formality metric reveals that dementia patients create samples of lower formality levels. When computing the correlation matrices we observe that it is negatively correlated with the label class as well ($r$ =$-0.26$ for ADR | $r$ =$-0.14$ for DB). Similarly, the complexity score is lower for AD. 
We find that as expected the class shows signs of lower fluency (higher \emph{INTJ} and \emph{EDIT count}, lower rates of subject \& verbs (\emph{S\&V}) sentences and sentences starting with a subject (\emph{ROOT$\rightarrow$S})). Surprisingly, the AD samples show lower frequencies of nouns without determinants than the control class. Although the mean perplexity scores are lower for the CC class, both the correlation and significance are weak. Our metrics related to wordiness also indicate that indeed AD patients use more adverbs, pronouns and verbs to compensate for the lack of specific nouns. These sets of metrics (PR/NOUN, ADV/NOUN and V/NOUN)  are also highly correlated with the label class on the ADReSS dataset and similarly PR/NOUN metrics on the DementiaBank dataset. On both datasets, the sentence length metric indicates that AD samples are shorter.
We also observe that formality is correlated with multiple metrics encompassing fluency ( -0.26 | -0.11,  | -0.07  for INTJ \& EDIT) and complexity.

These findings indicate that there are significant structural differences in terms of sentences between dementia and control speech. Text standardization can convert both dementia and control sentences to conform to the same structural standards. Therefore we hypothesize that \textit{text standardization can help conceal dementia in transcribed speech}.

==> Sections/qualitative_analysis.tex <==






